Algebraic Algorithms for b-Matching, Shortest Undirected Paths, and f-Factors

Let G=(V,E) be a graph with f:V\to Z_+ a function assigning degree bounds to vertices. We present the first efficient algebraic algorithm to find an f-factor. The time is \tilde{O}(f(V)^{\omega}). More generally for graphs with integral edge weights of maximum absolute value W we find a maximum weight f-factor in time \tilde{O}(Wf(V)^{\omega}). (The algorithms are randomized, correct with high probability and Las Vegas; the time bound is worst-case.) We also present three specializations of these algorithms: For maximum weight perfect f-matching the algorithm is considerably simpler (and almost identical to its special case of ordinary weighted matching). For the single-source shortest-path problem in undirected graphs with conservative edge weights, we present a generalization of the shortest-path tree, and we compute it in \tilde{O(Wn^{\omega}) time. For bipartite graphs, we improve the known complexity bounds for vertex capacitated max-flow and min-cost max-flow on a subclass of graphs.

==> apendix-allowed.tex <==
We define {\em allowed edge} to be an edge belonging to some $f$-factor. In case of perfect matchings
 the notion of allowed edge is easily expressible using inverse matrix of $B$. It can be shown that
 an edge $ij$ is allowed if and only if $B^{-1}_{i,j}$ is non-zero~\cite{rv89}. The next lemma shows
 why similar statement is not true for general $f$-factor. First, for $f$ let us define $f_{i,j}$ to be
\[
f_{i,j}(v) = \begin{cases}
f(v) & \mathrm{if } v \neq i,j,\\
f(v)-1 & \mathrm{otherwise.}
\end{cases}
\]

\begin{lemma}
\label{lemma:f_i_j-factor}
Let $G$ be a bipartite graph having an $f$-factor and let $B=B(G)$ be its symbolic adjacency matrix.
Consider two vertices $i\in V_0$ and $j \in V_1$, such that $f(i)>0$ and $f(j)>0$. Then $(B^{-1})_{n(j),n(i)}\neq 0$ if and
only if $G$ has $f_{i,j}$-factor.
\end{lemma}
\begin{proof}
Observe that
\[
(B^{-1})_{n(j),n(i)} = \frac{(-1)^{n(i)+n(j)}\det(B^{n(i),n(j)})}{\det(B)},
\]
where $B^{n(i),n(j)}$ is the matrix $B$ with $n(i)$'th row and $n(j)$'th column removed. We know that $\det(B)\neq 0$, because $G$ has $f$-factor. Hence, $(B^{-1})_{n(j),n(i)}\neq 0$ if and only if $\det(B^{n(i),n(j)}) \neq 0$. However, $B^{n(i),n(j)}$ is the symbolic adjacency matrix
obtained from $G$ for $f_{i,j}$ factor.
\end{proof}

\begin{figure}[h]
\centering
  \includegraphics[width=0.5\textwidth]{f_i_j-factor.eps}
\caption{The only $2$-factor is shown on panel a), whereas the only $f_{u,v}$-factor is shown on panel b). Edge $uv$ is not allowed
in any $2$-factor, although $f_{u,v}$-factor does exist.}
\label{figure:f_i_j-factor}
\end{figure}

Observe that for any edge $ij$ as long as $f(i)=f(j)=1$ the existence of $f_{i,j}$-factor is equivalent to the fact that $ij$ is allowed. However,
as shown on Figure~\ref{figure:f_i_j-factor}, the edge $uv$ is not allowed, although the $f_{u,v}$-factor does exit. The reason for this is that
we are trying to use edge $uv$ twice. The right criteria that follows directly from Lemma~\ref{lemma:f_i_j-factor} is given by the next corollary.

\begin{corollary}
Let $G$ be a bipartite graph having an $f$-factor. The edge $ij \in E(G)$ is allowed if and only if $(B(G-ij)^{-1})_{n(j),n(i)}\neq 0$.
\end{corollary}

The above corollary shows that in order to find the $f$-factor, we would need to combine Gaussian elimination with matrix updates.

==> bipartite-algorithms-0.tex <==
\subsection{Finding $f$-factors}
\label{section:biparite:algorithms}

This section gives our algorithm to find an $f$-factor of
a  bipartite multigraph. We follow the
development from~\cite{ms04}:
We start with  an $O(\phi^3)$-time algorithm. Then we show
it can be implemented in $O(\phi^{\omega})$ time using the fast
Gaussian elimination algorithm of Bunch and Hopcroft~\cite{hb}.

An {\em allowed edge} is an edge belonging to some $f$-factor. 
For perfect matchings
the notion of allowed edge is easily expressible using the
inverse of $B(G)$:
$ij$ is allowed if and only if $B(G)^{-1}_{i,j}$ is non-zero~\cite{rv89}. 
We will prove a similar
statement for bipartite $f$-factors.
(But such a statement fails for
non-bipartite graphs -- see Appendix~\ref{appendix-allowed-edges}.)
First, for $f$ define $f_{i,j}$ to be
\[
f_{i,j}(v) = \begin{cases}
f(v)-1 & \textrm{if } v = i \textrm{ or } v=j,\\
f(v) & \textrm{otherwise.}
\end{cases}
\]
\begin{lemma}
Let $G$ be a bipartite multigraph having an $f$-factor. Edge $ij\in E$ is
allowed if and only if $G$ has an $f_{i,j}$-factor.
\end{lemma}
\begin{proof}
%TODO rysunek
The ``only if'' direction is clear:
If $F$ is an $f$-factor containing
$ij$, then $F-ij$ is an $f_{i,j}$-factor.

Conversely, suppose $F$ does not contain
the chosen edge $ij$. Take any $f_{i,j}$-factor $F'$ in $G$.
$F'\oplus F$ contains an 
alternating $ij$-path $P$ 
that starts and ends with edges of $F$.
So $ij$ is not the first edge of $P$.
In fact $ij\notin P$, since $P$ is vertex simple.  
(In proof,
any cycle in $P$
has even length, so it can be discarded
to get a shorter alternating path.) 
Thus $(F\oplus P) +ij$ is an $f$-factor containing $ij$.
\end{proof}

Conversely,
take any $f_{i,j}$-factor $F'$ in $G$. 
If $F'$ does not use all the copies of the edge $ij$ 
then $F'+ij$ is the desired $f$-factor. So assume
$F'$ uses every copy of $ij$. 
Let $F$ be any $f$-factor in $G$. 
We note that $F'-ij$ (i.e., $F'$ with one copy of edge $ij$ removed) 
is and $(f_{i,j})_{i,j}$-factor. Hence, $F\oplus (F'-ij)$ needs
to contain two augmenting alternating path with respect to $F'$. These paths need to start in $i$ and end in $j$.~\footnote{In non-bipartite case
one path could start and end in $i$, whereas the other one could start and end in $j$.} Let $P$ be one of these paths, then
$F'\oplus P$ is an $f$-factor that contains edge $ij$.


\begin{lemma}
\label{lemma:f_i_j-factor}
Let $G$ be a bipartite multigraph having an $f$-factor, let $B(G)$ be its symbolic adjacency matrix, and let $i\in V_0$ and $j \in V_1$.
Then $(B(G)^{-1})_{j,0,i,0}\neq 0$ if and only if $G$ has $f_{i,j}$-factor.
\end{lemma}
\begin{proof}
Observe that
\[
(B(G)^{-1})_{j,0,i,0} = \frac{(-1)^{n(j,0)+n(i,0)}\det(B(G)^{i,0,j,0})}{\det(B(G))},
\]
where $B(G)^{i,0,j,0}$ is the matrix $B(G)$ with $i,0$'th row and $j,0$'th column removed, and $n(i,k)$ is the
actual index of the row or column given be the pair $i,k$. We know that $\det(B(G))\neq 0$, because $G$ has an $f$-factor. Hence, $(B(G)^{-1})_{j,0,i,0}\neq 0$
if and only if $\det(B(G)^{i,0,j,0}) \neq 0$. However, $B(G)^{i,0,j,0}$ is the symbolic adjacency matrix
obtained from $G$ for $f_{i,j}$-factors.
\end{proof}

Combining the above two lemmas we obtain the following.

\begin{corollary}
\label{corollary:allowed-edge}
Let $G$ be a bipartite multigraph having an $f$-factor, and let $B(G)$ be its symbolic adjacency matrix. The edge $ij\in E$ is
allowed if and only if $(B(G)^{-1})_{j,0,i,0}\neq 0$.
\end{corollary}

%Let $e=ij \in E(G)$ then $B(G)$ and $B(G-e)$ differ from one another by a rank-one update, i.e.,
%\[
%B(G-e) = B(G) - x_{i}^e (y_j^e)^T
%\]
%where $x_{i}^e$ and $y_j^e$ are length $\phi$ vectors defines as
%\begin{eqnarray*}
%(x_{i}^e)_k = \begin{cases}
%x_{i,r-n(i)}^e & \textrm{if } n(i) \le k <n(i)+f(i),\\
%0 & \textrm{otherwise,}
%\end{cases} & \textrm{ and } &
%(y_{j}^e)_k = \begin{cases}
%y_{j,r-n(j)}^e & \textrm{if } n(j) \le k <n(j)+f(j),\\
%0 & \textrm{otherwise.}
%\end{cases}
%\end{eqnarray*}

Being equipped with a tool for finding allowed edges we can use the following algorithm for finding $f$-factors.

\begin{algorithm}[H]
\caption{An $O(\phi^3)$ time algorithm for finding $f$-factor in bipartite multigraph $G$.}
\begin{algorithmic}[1]
\State{Let $B(G)$ be $\phi \times \phi$ matrix representing $G$}
\State{Replace the variables in $B(G)$ for random elements from $\mathcal{Z}_p$ for prime $p=\Theta(\phi^2)$ to obtain $B$}
\State{If $B$ is singular return "no $f$-factor"}
\State{(with probability $\ge 1-\frac{1}{\phi}$ matrix $B$ is non-singular when $B(G)$ is non-singular)}\comment{by
Lemma~\ref{corollary-zippel-schwartz}}
\State{$F=\emptyset$}
\State{Compute $B^{-1}$}
\State{($\det(B)\neq 0$ so in each row and column of $B^{-1}$ there is an nonzero element, i.e., allowed edge)}
%\comment{by Lemma~\ref{corollary-zippel-schwartz}}
\For{$i=[1..n]$}
\For{$\iota=[0..f(i)-1]$}
\State{Find $j$ such that $ij \in E$ and $B^{-1}_{j,\iota,i,\iota}\neq 0$}\comment{by Corollary~\ref{corollary:allowed-edge} edge $ij$ is allowed}
\State{Eliminate the $j,\iota$'th row and the $i,\iota$'th column from $B^{-1}$}\comment{using Gaussian elimination}
\label{algorithm:f-factor-bipartite-simple:eliminate}
%\State \comment{Equivalently we can zero out all element in $j,\iota$th row and the $i,\iota$th column, besides $N_{j,\iota,i,\iota}$}
\State{Set $F:=F+ij$}
\EndFor
\EndFor
\State{Return $F$}
%\EndProcedure
\end{algorithmic}
\label{algorithm:f-factor-bipartite-multi}
\end{algorithm}

It might be easier to think of line~\ref{algorithm:f-factor-bipartite-simple:eliminate} in the
following way: set elements in $i,\iota$'th row and the $j,\iota$'th column of $B$ to 0, but keep $B_{i,\iota,j,\iota}$ unchanged;
update $B^{-1}$ accordingly to this change using Sherman-Morrison formula. Nevertheless, you might notice
that we are implementing Gaussian elimination on $B^{-1}$ with the only difference that pivoting points are chosen in such a way that
they correspond to edges. Hence, one can implement this algorithm to work in $O(\phi^{\omega})$ time using the ideas of Bunch and Hopcroft~\cite{hb}.

\paragraph{Generalizations}
Section~\ref{sec:algorithms} gives $O(\phi^{\omega})$ time algorithms for finding $f$-factors in non-bipartite multigraphs. There are
several things that need to be done differently. As discussed above the criteria for finding allowed edges -- Corollary~\ref{corollary:allowed-edge} does not work any more. We need to work with weaker notion of {\em removable edges}, i.e.,
the edges that can be removed from the graph so that it still contains an $f$-factor. This forces us to use different approach,
based on Harvey~\cite{Harvey06}, which works with removable edges. This posses a new challenge to handle multiple copies
of edges in multi-graphs, as removing such edges one by one could require $O(\phi^3)$ time. To overcome this problem we use binary search with
Sherman-Morrison-Woodbory formula to remove multiple copies of an edge in one shot. 


==> bipartite-algorithms-1.tex <==
\subsection{Finding $f$-factors}
\label{section:biparite:algorithms}

This section gives our algorithm to find an $f$-factor of
a  bipartite multigraph. We follow the
development from~\cite{ms04}:
We start with  an $O(\phi^3)$-time algorithm. Then we show
it can be implemented in $O(\phi^{\omega})$ time using the fast
Gaussian elimination algorithm of Bunch and Hopcroft~\cite{hb}.

An {\em allowed edge} is an edge belonging to some $f$-factor.
For perfect matchings
the notion of allowed edge is easily expressible using the
inverse of $B(G)$:
$ij$ is allowed if and only if $B(G)^{-1}_{i,j}$ is non-zero~\cite{rv89}.
We will prove a similar
statement for bipartite $f$-factors.
(But such a statement fails for
non-bipartite graphs -- see Appendix~\ref{appendix-allowed-edges}.)
First, for $f$ define $f_{i,j}$ to be
\[
f_{i,j}(v) = \begin{cases}
f(v)-1 & \textrm{if } v = i \textrm{ or } v=j,\\
f(v) & \textrm{otherwise.}
\end{cases}
\]
\begin{lemma}
Let $G$ be a bipartite multigraph having an $f$-factor. Edge $ij\in E$ is
allowed if and only if $G$ has an $f_{i,j}$-factor.
\end{lemma}
\begin{proof}
%TODO rysunek
The ``only if'' direction is clear:
If $F$ is an $f$-factor containing
$ij$, then $F-ij$ is an $f_{i,j}$-factor.

Conversely, suppose $F$ does not contain
the chosen edge $ij$. Take any $f_{i,j}$-factor $F'$ in $G$.
$F'\oplus F$ contains an
alternating $ij$-path $P$
that starts and ends with edges of $F$.
So $ij$ is not the first edge of $P$.
In fact $ij\notin P$, since $P$ is vertex simple.
(In proof,
any cycle in $P$
has even length, so it can be discarded
to get a shorter alternating path.)
Thus $(F\oplus P) +ij$ is an $f$-factor containing $ij$.
\end{proof}


\begin{lemma}
\label{lemma:f_i_j-factor}
Let $G$ be a bipartite multigraph having an $f$-factor, let $B(G)$ be its symbolic adjacency matrix, and let $i\in V_0$ and $j \in V_1$.
Then $(B(G)^{-1})_{j,0,i,0}\neq 0$ if and only if $G$ has $f_{i,j}$-factor.
\end{lemma}
\begin{proof}
Observe that
\[
(B(G)^{-1})_{j,0,i,0} = \frac{(-1)^{n(j,0)+n(i,0)}\det(B(G)^{i,0,j,0})}{\det(B(G))},
\]
where $B(G)^{i,0,j,0}$ is the matrix $B(G)$ with $i,0$'th row and $j,0$'th column removed, and $n(i,k)$ is the
actual index of the row or column given by the pair $i,k$. We have $\det(B(G))\neq 0$ since $G$ has an $f$-factor. Hence $(B(G)^{-1})_{j,0,i,0}\neq 0$
if and only if $\det(B(G)^{i,0,j,0}) \neq 0$. Furthermore $B(G)^{i,0,j,0}$ is the symbolic adjacency matrix
obtained from $G$ for $f_{i,j}$-factors.
\end{proof}

Combining the above two lemmas we obtain the following.

\begin{corollary}
\label{corollary:allowed-edge}
Let $G$ be a bipartite multigraph having an $f$-factor, and let $B(G)$ be its symbolic adjacency matrix. The edge $ij\in E$ is
allowed if and only if $(B(G)^{-1})_{j,0,i,0}\neq 0$.
\end{corollary}

%Let $e=ij \in E(G)$ then $B(G)$ and $B(G-e)$ differ from one another by a rank-one update, i.e.,
%\[
%B(G-e) = B(G) - x_{i}^e (y_j^e)^T
%\]
%where $x_{i}^e$ and $y_j^e$ are length $\phi$ vectors defines as
%\begin{eqnarray*}
%(x_{i}^e)_k = \begin{cases}
%x_{i,r-n(i)}^e & \textrm{if } n(i) \le k <n(i)+f(i),\\
%0 & \textrm{otherwise,}
%\end{cases} & \textrm{ and } &
%(y_{j}^e)_k = \begin{cases}
%y_{j,r-n(j)}^e & \textrm{if } n(j) \le k <n(j)+f(j),\\
%0 & \textrm{otherwise.}
%\end{cases}
%\end{eqnarray*}

Being equipped with a tool for finding allowed edges we can use the following algorithm 
to find an $f$-factor. 

\begin{algorithm}[H]
\caption{An $O(\phi^3)$ time algorithm to find an $f$-factor in a bipartite multigraph $G$.}
\begin{algorithmic}[1]
\State{Let $B(G)$ be the $\phi \times \phi$ matrix representing $G,f$}
\State{Replace the variables in $B(G)$ by random values from $\mathcal{Z}_p$ for prime $p=\Theta(\phi^2)$ to obtain $B$}
\State{If $B$ is singular return "no $f$-factor"}
\State{(with probability $\ge 1-\frac{1}{\phi}$ matrix $B$ is non-singular when $B(G)$ is non-singular)}\comment{by
Cor.~\ref{corollary-zippel-schwartz}}
\State{$F=\emptyset$}
\State{Compute $B^{-1}$}
\State{($\det(B)\neq 0$ so each row and column of $B^{-1}$ has a nonzero element, i.e., an allowed edge)}
%\comment{by Lemma~\ref{corollary-zippel-schwartz}}
\For{$i=[1..n]$}
\For{$\iota=[0..f(i)-1]$}
\State{Find $j$ such that $ij \in E$ and $B^{-1}_{j,\iota,i,\iota}\neq 0$}\comment{by Corollary~\ref{corollary:allowed-edge} edge $ij$ is allowed}
\State{Eliminate the $j,\iota$'th row and the $i,\iota$'th column from $B^{-1}$}\comment{using Gaussian elimination}
\label{algorithm:f-factor-bipartite-simple:eliminate}
%\State \comment{Equivalently we can zero out all element in $j,\iota$th row and the $i,\iota$th column, besides $N_{j,\iota,i,\iota}$}
\State{Set $F:=F+ij$}
\EndFor
\EndFor
\State{Return $F$}
%\EndProcedure
\end{algorithmic}
\label{algorithm:f-factor-bipartite-multi}
\end{algorithm}

One can think of line~\ref{algorithm:f-factor-bipartite-simple:eliminate} in the
following way: Set every element in row $i,\iota$ or column $j,\iota$ of $B$ to 0 except  for $B_{i,\iota,j,\iota}$, which is unchanged;
then update $B^{-1}$ according to this change using the Sherman-Morrison formula. This equivalence results from the properties of Schur complement. 
In other words 
line~\ref{algorithm:f-factor-bipartite-simple:eliminate} computes $B^{-1}$ for an $f_{i,j}$-factor.
Notice
that we are implementing Gaussian elimination on $B^{-1}$, the only difference being that pivot elements are chosen to
correspond to edges. If there exists an $f$-factor, there is an allowed edge incident to each vertex. 
Hence, even with this additional requirement Gaussian elimination is able to find a non-zero element in each row of $B^{-1}$.

Bunch and Hopcroft~\cite{hb} show how to speed up the running time of Gaussian elimination 
from $O(\phi^3)$ to $O(\phi^{\omega})$, by using lazy updates to the matrix. Let us divide the columns of 
the matrix into two equal halves $L$ and $R$ according to the order in which they appear in the matrix. 
 Bunch and Hopcroft observe that columns in $R$ are not used until we eliminate all columns from $L$. 
Hence all  updates to columns in $R$ resulting from elimination of columns in $L$ can be done once
using fast matrix multiplication in $O(|R|^{\omega})$ time. By applying this scheme 
recursively one obtains an $O(\phi^{\omega})$ time algorithm. 

\paragraph{Generalizations}
Section~\ref{sec:algorithms} gives $O(\phi^{\omega})$ time algorithms for finding $f$-factors in non-bipartite multigraphs. There are
several things that need to be done differently. As discussed above the criteria for finding allowed edges -- Corollary~\ref{corollary:allowed-edge} -- does not work any more. 
We need to work with the weaker notion of {\em removable edges}, i.e.,
the edges that can be removed from the graph so that it still contains an $f$-factor. This forces us to use a different approach,
based on Harvey~\cite{Harvey06}, which works with removable edges. This poses a new challenge, to handle multiple copies
of edges in multi-graphs, as removing such edges one by one could require $O(\phi^3)$ time. To overcome this problem we use binary search with the
Sherman-Morrison-Woodbury formula to remove multiple copies of an edge in one shot.


==> bipartite-algorithms-2.tex <==
\subsection{Finding $f$-factors}
\label{section:biparite:algorithms}

This section gives our algorithm to find an $f$-factor of
a  bipartite multigraph. We follow the
development from~\cite{ms04}:
We start with  an $O(\phi^3)$-time algorithm. Then we show
it can be implemented in $O(\phi^{\omega})$ time using the fast
Gaussian elimination algorithm of Bunch and Hopcroft~\cite{hb}.

An {\em allowed edge} is an edge belonging to some $f$-factor.
For perfect matchings
the notion of allowed edge is easily expressible using the
inverse of $B(G)$:
$ij$ is allowed if and only if $B(G)^{-1}_{i,j}$ is non-zero~\cite{rv89}.
We will prove a similar
statement for bipartite $f$-factors.
(But such a statement fails for
non-bipartite graphs -- see Appendix~\ref{appendix-allowed-edges}.)
First, for $f$ define $f_{i,j}$ to be
\[
f_{i,j}(v) = \begin{cases}
f(v)-1 & \textrm{if } v = i \textrm{ or } v=j,\\
f(v) & \textrm{otherwise.}
\end{cases}
\]
\begin{lemma}
Let $G$ be a bipartite multigraph having an $f$-factor. Edge $ij\in E$ is
allowed if and only if $G$ has an $f_{i,j}$-factor. Additionally, 
if edge $ik\in E$, belongs to some $f_{i,j}$-factor in $G$ then it is allowed
in $G$. 
\end{lemma}
\begin{proof}
%TODO rysunek
The ``only if'' direction is clear:
If $F$ is an $f$-factor containing
$ij$, then $F-ij$ is an $f_{i,j}$-factor.

Conversely, suppose $F$ does not contain
the chosen edge $ij$. Take any $f_{i,j}$-factor $F'$ in $G$.
$F'\oplus F$ contains an
alternating $ij$-path $P$
that starts and ends with edges of $F$.
So $ij$ is not the first edge of $P$.
In fact $ij\notin P$, since $P$ is vertex simple.
(In proof,
any cycle in $P$
has even length, so it can be discarded
to get a shorter alternating path.)
Thus $(F\oplus P) +ij$ is an $f$-factor containing $ij$.

Assume now that $F'$ uses edge $ik$. Observe that path $P$ 
cannot contain edge $ik$ because it is vertex simple and
starts with edges of $F$. Hence, $(F\oplus P)+ij$ is 
an $f$-factor containing both $ij$ and $ik$. 
\end{proof}


\begin{lemma}
\label{lemma:f_i_j-factor}
Let $G$ be a bipartite multigraph having an $f$-factor, let $B(G)$ be its symbolic adjacency matrix, and let $i\in V_0$ and $j \in V_1$.
Then $(B(G)^{-1})_{j,0,i,0}\neq 0$ if and only if $G$ has $f_{i,j}$-factor.
\end{lemma}
\begin{proof}
Observe that
\[
(B(G)^{-1})_{j,0,i,0} = \frac{(-1)^{n(j,0)+n(i,0)}\det(B(G)^{i,0,j,0})}{\det(B(G))},
\]
where $B(G)^{i,0,j,0}$ is the matrix $B(G)$ with $i,0$'th row and $j,0$'th column removed, and $n(i,k)$ is the
actual index of the row or column given by the pair $i,k$. We have $\det(B(G))\neq 0$ since $G$ has an $f$-factor. Hence $(B(G)^{-1})_{j,0,i,0}\neq 0$
if and only if $\det(B(G)^{i,0,j,0}) \neq 0$. Furthermore $B(G)^{i,0,j,0}$ is the symbolic adjacency matrix
obtained from $G$ for $f_{i,j}$-factors.
\end{proof}
Observe that by the symmetry of the matrix $B(G)$, when $(B(G)^{-1})_{j,0,i,0}\neq 0$ then as 
well $(B(G)^{-1})_{j,\iota,i,\kappa}\neq 0$ for all $0\le \iota <f(i)$ and $0\le \kappa <f(j)$. 
Combining the above two lemmas with this observation we obtain the following.

\begin{corollary}
\label{corollary:allowed-edge}
Let $G$ be a bipartite multigraph having an $f$-factor, and let $B(G)$ be its symbolic adjacency matrix. The edge $ij\in E$ is
allowed if and only if $(B(G)^{-1})_{j,\iota,i,\kappa }\neq 0$ for any $0\le \iota <f(i)$ and $0\le \kappa <f(j)$.
\end{corollary}

%Let $e=ij \in E(G)$ then $B(G)$ and $B(G-e)$ differ from one another by a rank-one update, i.e.,
%\[
%B(G-e) = B(G) - x_{i}^e (y_j^e)^T
%\]
%where $x_{i}^e$ and $y_j^e$ are length $\phi$ vectors defines as
%\begin{eqnarray*}
%(x_{i}^e)_k = \begin{cases}
%x_{i,r-n(i)}^e & \textrm{if } n(i) \le k <n(i)+f(i),\\
%0 & \textrm{otherwise,}
%\end{cases} & \textrm{ and } &
%(y_{j}^e)_k = \begin{cases}
%y_{j,r-n(j)}^e & \textrm{if } n(j) \le k <n(j)+f(j),\\
%0 & \textrm{otherwise.}
%\end{cases}
%\end{eqnarray*}

Being equipped with a tool for finding allowed edges we can now use the framework from~\cite{ms04}. 
The following observation is useful. 
\begin{lemma}[\cite{ms04}]
\label{lemma-elimination}
Let $A$ be a non-singular $\phi \times \phi$ matrix and let $1\le i,j \le n$ be such that $A^{-1}_{j,i} \neq 0$. 
Let $A'$ be the matrix obtained from $A^{-1}$ by eliminating row $j$ and column $i$ using Gaussian elimination, then
$A'= (A^{i,j})^{-1}$ (i.e., $A'$ is the Schur compliment of $(A^{-1})^{j,i}$). 
\end{lemma}

The above lemma can be used to obtain the following algorithm that finds an $f$-factor.

\begin{algorithm}[H]
\caption{An $O(\phi^3)$ time algorithm to find an $f$-factor in a bipartite multigraph $G$.}
\begin{algorithmic}[1]
\State{Let $B(G)$ be the $\phi \times \phi$ matrix representing $G,f$}
\State{Replace the variables in $B(G)$ by random values from $\mathcal{Z}_p$ for prime $p=\Theta(\phi^2)$ to obtain $B$}
\State{If $B$ is singular return "no $f$-factor"}
\State{(with probability $\ge 1-\frac{1}{\phi}$ matrix $B$ is non-singular when $B(G)$ is non-singular)}\comment{by
Cor.~\ref{corollary-zippel-schwartz}}
\State{$F=\emptyset$}
\State{Compute $N=B^{-1}$}
\State{($\det(B)\neq 0$ so each row and column of $B^{-1}$ has a nonzero element, i.e., an allowed edge)}
%\comment{by Lemma~\ref{corollary-zippel-schwartz}}
\For{$i=[1..n]$}
\For{$\iota=[0..f(i)-1]$}
\State{Find $j$ such that $ij \in E\ominus F$  and $N_{j,\iota,i,\iota}\neq 0$}\comment{by Corollary~\ref{corollary:allowed-edge} edge $ij$ is allowed}
\State{Eliminate the $j,\iota$'th row and the $i,\iota$'th column from $N$}\comment{using Gaussian elimination}
\State{(by Lemma~\ref{lemma-elimination} we have $N=(B^{i,\iota,j,\iota})^{-1}$, i.e., $N$ encodes $f_{i,j}$-factors)}
\label{algorithm:f-factor-bipartite-simple:eliminate}
%\State \comment{Equivalently we can zero out all element in $j,\iota$th row and the $i,\iota$th column, besides $N_{j,\iota,i,\iota}$}
\State{Set $F:=F\oplus ij$}
\EndFor
\EndFor
\State{Return $F$}
%\EndProcedure
\end{algorithmic}
\label{algorithm:f-factor-bipartite-multi}
\end{algorithm}

Observe that in the above algorithm we are implementing Gaussian elimination on $B^{-1}$, the only difference being that pivot elements are chosen to
correspond to edges. If there exists an $f$-factor, there is an allowed edge incident to each vertex.
Hence, even with this additional requirement Gaussian elimination is able to find a non-zero element in each row of $B^{-1}$.

Bunch and Hopcroft~\cite{hb} show how to speed up the running time of Gaussian elimination
from $O(\phi^3)$ to $O(\phi^{\omega})$, by using lazy updates to the matrix. Let us divide the columns of
the matrix into two almost equal parts. Let $L$ denote the first $\lceil \phi/2 \rceil$ 
columns that are to be eliminated, whereas let $R$ denote the remaining $\lfloor \phi/2 \rfloor$ columns.  
Bunch and Hopcroft observed that columns in $R$ are not used until we eliminate all columns from $L$.\footnote{In their paper 
the elimination proceeds row by row, whereas it is nowadays more usual to present Gaussian elimination on columns.}
Hence all  updates to columns in $R$ resulting from elimination of columns in $L$ can be done once
using fast matrix multiplication in $O(|R|^{\omega})$ time. By applying this scheme
recursively one obtains an $O(\phi^{\omega})$ time algorithm.

\paragraph{Generalizations}
Section~\ref{sec:algorithms} gives $O(\phi^{\omega})$ time algorithms for finding $f$-factors in non-bipartite multigraphs. There are
several things that need to be done differently. As discussed above the criteria for finding allowed edges -- Corollary~\ref{corollary:allowed-edge} -- does not work any more.
We need to work with the weaker notion of {\em removable edges}, i.e.,
the edges that can be removed from the graph so that it still contains an $f$-factor. This forces us to use a different approach,
based on Harvey~\cite{Harvey06}, which works with removable edges. This poses a new challenge, to handle multiple copies
of edges in multi-graphs, as removing such edges one by one could require $O(\phi^3)$ time. To overcome this problem we use binary search with the
Sherman-Morrison-Woodbury formula to remove multiple copies of an edge in one shot.


==> determinant-old0.tex <==
\section{Determinant formulations for general graphs}
\label{sec:determinant}
Let $G$ be a simple graph with vertices numbered from 1 to $n$.
Let $\phi=\sum_i f(i)$. We
define a skew-symmetric $\phi \times \phi$ matrix $B(G)$ representing $G$ in the following
way. A vertex $i\in V$ is associated with
$f(i)$ consecutive rows and columns of $B$ numbered by pairs $i,r$, for $0\le r<f(i)$.
We call a tuple $(i,r,j,c)$ representing the entry $B(G)_{i,r,j,c}$
{\it permissible} if either
\[i<j, %
\text{ or } i=j \text{ and } r<\f{f(i)/2}\le \c{f(i)/2}\le c<f(i).
\]
The set of permissible entries is denoted by $\mathbb P$.
Note that the permissible entries of $B(G)$ are all above the diagonal.
The permissible entries corresponding to a fixed edge $e$
form  a
rectangular submatrix for a nonloop $e$ and 
an $\f{f(i)/2} \times \f{f(i)/2}$ submatrix for a loop $ii$.

Using indeterminates $x^{ij}_{r}$, $y^{ij}_{c}$ we define an entry of $B(G)$ as
\begin{equation}
\label{SimpleGenMatrixEqn}
B(G)_{i,r,j,c} \!=\!
\begin{cases}
x^{ij}_{r} y^{ij}_{c}& %
ij\!\in\! E \text{ and } (i,r,j,c)\in \mathbb P,\\ % \text{ is permissible,}\cr
-x^{ji}_{c} y^{ji}_{r}&  %
ij\! \in\! E \text{ and } (j,c, i,r)\in \mathbb P,\\ % \text{ is permissible,}\cr
0&\text{otherwise.}
\vspace{-0.1cm}
\end{cases}
\end{equation}
Clearly $B(G)$ is skew-symmetric. Note that a loop $ii\in E$ is represented by
an $\f{f(i)/2}\times \f{f(i)/2}$ submatrix that is empty
if $f(i)=1$. This is fine since $ii$ is not in any $f$-factor.



We shall use some simple relations between $G$ and terms of $\det(B(G))$.
Recall that any permutation is a product of cyclic permutations.
A permutation $\pi$ containing the cyclic permutation  $(i_1 i_2 \ldots i_k)$
can be associated with another permutation $\pi'$ that is identical to $\pi$
except that the cycle is reversed to $(i_k\ldots i_2 i_1)$.
$\pi$ and $\pi'$ have the same sign. When $\pi$ specifies a term in the expansion
of a determinant, $\pi'$ specifies the term that is identical except that the entries for
the cycle are transposed.

Now consider
a term $\sigma$ of $\det(B(G))$ and its associated permutation $\pi$.
Remembering that each entry in $B(G)$ corresponds to an edge of $G$,
we see that 
each cycle of $\pi$ gives a corresponding cycle of $G$.
Reversing a cycle of $\pi$ transposes the entries of $\sigma$, as above. Each transposed entry has the same variables and opposite sign. 
So an even (odd) cycle of $G$ gives a new term  exactly equal to 
$\sigma$ ($-\sigma$), respectively.

Every nonzero entry of $B(G)$ corresponds to an edge of $G$, so a term
$\sigma$ in the expansion of $\det(B(G))$ has a corresponding subgraph
$F_\sigma$. $F_\sigma$ is unique (since each indeterminate, e.g.~$x^{ij}_r$, specifies its edge).
$F_\sigma$ has $\phi$ edges. In fact
each vertex $i$ has degree $2f(i)$. So
$F_{\sigma}$ is a $2f$-factor.
$F_\sigma$ may contain many copies of
a given edge, coming from entries of $B(G)$ both above and below the diagonal.
As observed above, the edges of $F_\sigma$ are partitioned into cycles by the permutation
$\pi$ of $\sigma$. (Viewed simply as a set of edges, $F_\sigma$ 
may be partitioned into cycles
in perhaps more than one way. However we will always use the partition induced by $\pi$.)

Any $f$-factor $F$ of $G$ gives the $2f$-factor $2F$
of $2G$. Various terms $\sigma$ in the expansion of $\det(B(G))$
have $F_\sigma=2F$. Such terms use two corresponding entries for each of its edges, i.e.,
ignoring sign $\sigma$ is a product of
$\phi/2$ terms of the form $(x^{ij}_{r} y^{ij}_{c})^2$.
(Since indices $r$ and $c$ for edge $ij$ can vary,
more than one term may correspond to $2F$.)
Clearly  $F_\sigma/2$ is an $f$-factor.
We will show that $\det(B(G))$ includes all such terms $\sigma$, but also
other terms that correspond to sums of two different $f$-factors. 

\def\FF.{\Phi_2(G)}%formerly \F._2(G) , but this is too much like \F.(G)

As before
define $\F.$ to be the function that maps each term $\sigma$ to $F_{\sigma}$;
the difference is that now $F_{\sigma}$ is a $2f$-factor.
Let $\FF.$ be the set
formed by taking sums of two 
(possibly equal) $f$-factors of $G$, i.e.,
\[
%\F._2(G) = \sum_{F_1, F_2: \textrm{$f$-factor of } G} F_1 \uplus F_2,
\FF.=
\{F_1 \uplus F_2: F_1, F_2\textrm{ $f$-factors of } G\} .
\]
Here $\uplus$ denotes multiset sum.


\iffalse
As before
define $\F.$ to be the function that maps each term $\sigma$ to $F_{\sigma}$;
the difference is that now $F_{\sigma}$ is a $2f$-factor.
Call two f-factors $F_1,F_2${\em similar} if $F_1\oplus F_2$ does not
contain an alternating cycle $C$ of odd length (i.e., traversing
$C$, the edges alternate between $F_1$ and $F_2$, except at the
vertex that starts and ends $C$).
Let $\FF.$ be the set
formed by taking sums of two 
similar $f$-factors of $G$, i.e.,
\[
%\F._2(G) = \sum_{F_1, F_2: \textrm{$f$-factor of } G} F_1 \uplus F_2,
\FF.=
\{F_1 \uplus F_2: F_1, F_2\textrm{ similar $f$-factors of } G\} .
\]
Here $\uplus$ denotes multiset sum.
Note we can have $F_1=F_2$.
\fi


\begin{figure}[t]
\begin{center}
\resizebox{2.5in}{!}{\input {2triangles.pdf_t}}
\end{center}
\caption{Graph with 2 $f$-factors, $f(a)=2, f(v)=1$ for $v\ne a$..}

\label{NoPosetFig}
\end{figure}


\begin{theorem}
\label{GenSimpleDetThm}
Let $G$ be a simple graph. The function $\F.$ from terms in $\det(B(G))$ is
a surjection onto $\FF.$. Consequently, $G$ has an $f$-factor if and only if $\det(B(G))\ne 0$.
\end{theorem}
\begin{proof}

First let us show that the image of $\F.$ is contained in $\FF.$.
%Suppose that $\det(B(G))\ne 0$ and 
Consider a  term
$\sigma$ in the expansion of $\det(B(G))$.
As in the  bipartite case, $B(G)$ represents each edge  $ij$ by a rank-one submatrix given by an outer product
 $x^{ij} (y^{ij})^T$ ($i\le j)$. But now this submatrix appears twice, 
both above and below the diagonal and
with different sign. Thus
Lemma~\ref{lemma-submatrix} shows each edge $ij$ can be used at most
two times in $\sigma$.
Now we are left with two cases.
Both cases refer to the cycles of $F_\sigma$; recall that these are the cycles
uniquely determined by the permutation $\pi$ of $\sigma$.

\case {$F_\sigma$ consists of edges of multiplicity $\le 2$, and
contains an odd cycle of edges of multiplicity 1}

Associate $\sigma$ with the ordered pair $(i,j)$ where $i\le j$, edge
$ij$ belongs to an odd cycle of $\sigma$, and $(i,j)$ is lexically
minimum.  Pair $\sigma$ with the term $\sigma'$ that is identical to
$\sigma$ except its cycle containing $ij$ has the edges reversed.
As observed above $\sigma$ and $\sigma'$ have opposite sign.
Thus they cancel each other.

\iffalse
in opposite
orientation from $\sigma$ (i.e., $\sigma$ uses the entry for an edge
that is above the diagonal iff $\sigma'$ uses the entry below).  As permutations
$\sigma$ and $\sigma'$ have the same sign. Since
reversing an edge reverses the sign of the corresponding entry in $B(G)$ and the cycle is
odd, $\sigma$ and $\sigma'$ cancel each other.
\fi

\case {$F_\sigma$ consists of edges of multiplicity $2$, plus
edges of multiplicity 1 that are partitioned into even cycles}

The multiplicity 2 edges form length 2 cycles, so every edge is in
an even cycle of multiplicity 1 edges. Choosing alternate edges of each cycle
splits the $2f$-factor $F_\sigma$ into two $f$-factors.

\bigskip

Now we show that $\F.$ is surjective.
Let $F_1$ and $F_2$ be two $f$-factors. Observe that
connected components of $F_1 \uplus F_2$ are Eulerian. For each
component of $F_1 \uplus F_2$ construct an Eulerian tour. Orient each tour to obtain a directed set of tours $\sigma$.
However, we list each self-loop twice at the beginning of $\sigma$. We will show that this tour can be associated with a
term of $\det(B(G))$. Observe that for each vertex $v$ we have $f(v)$ outgoing edges, and $f(v)$ incoming edges.
We associate outgoing edges from $v$ with rows corresponding to $v$, whereas incoming are associated with columns
corresponding to $v$. We start by associating loops. The first copy of a loop $ii$ is
associated with 1'st row corresponding to $v$ and $f(v)-1$'th column corresponding to $v$, whereas the second copy is associated with
$f(v)-1$'th row and 1'st column. The remaining edges are associated in the order they appear
to the next free row and column associated with given vertex. In this way we construct a term that has a unique entry in each row,
as well as in each column. Moreover, observe that $F_1 \uplus F_2$ consists of edges of multiplicity $2$, plus
edges of multiplicity 1 that are partitioned into even cycles. Observe that no other term has exactly the same
indeterminates, so all such terms do not cancel with other terms.
\end{proof}

Now consider multigraphs. Let $\mu(e)$ denote the multiplicity of any edge $e$. Redefine $B(G)$ as
\begin{equation}
\label{MultiGenMatrixEqn}
B(G)_{i,r,j,c} =
\begin{cases}
{\sum _{k=1}^{\mu(e)} x^{ij,k}_{r} y^{ij,k}_{c}}& %
\minibox{$ij\in E$  and $(i,r,j,c) \in \mathbb P$,}\vspace{3pt}
 \\\vspace{3pt} %\text{ is permissible,}\cr
-\sum _{k=1}^{\mu(e)} x^{ij,k}_{c} y^{ij,k}_{r}&  %
\minibox{$ij \in E$  and  $(j,c, i,r) \in \mathbb P$,}\\% \text{ is permissible,}\cr
0&\text{otherwise.}
\end{cases}
\end{equation}

As in the case of bipartite multigraphs (compare with \eqref{MultiBipartiteMatrixEqn}) we
are now representing edge $ij$ by a submatrix of rank $\mu(ij)$. Thus
Lemma~\ref{lemma-submatrix} ensures that the edge $ij$ is used no more than 
a total of $2\mu(ij)$ times.
Hence, we obtain the following corollary.

\begin{corollary}
\label{GenMultiDetThm}
Let $G$ be a multigraph. The function $\F.$ from terms in $\det(B(G))$ is
a surjection onto $\FF.$. Consequently, $G$ has an $f$-factor if and only if $\det(B(G))\ne 0$.
\end{corollary}

%\begin{proof}
%The argument closely follows those of Theorem~\ref{GenSimpleDetThm}.  We just point out the small
%differences.
%
%First, we show that the image of $\F.$ is contained in $\F._2(G)$.
%Assume that $\det(B(G))\ne 0$.  We consider three types of terms
%$\sigma$.
%
%\case{$\sigma$ uses two entries of $B(G)$ for the same edge $e_k$ of $G$,
%both above the diagonal or both below the diagonal}
%
%We pair such terms $\sigma$ so they cancel, the same way as before,
%in two steps.
%
%First associate two duplicate entries with $\sigma$: form tuples $(e_k,\min\{r_1,r_2\}$, $\max\{r_1,r_2\}$,
%$\min\{c_1,c_2\}$, $\max\{c_1,c_2\})$ to assign the edge $e_k$ in $r_1c_1$, $r_2c_2$ to $\sigma$.
%
%Now the argument follows the theorem:
%If $\sigma$ is assigned the two entries $r_1 c_1$ and $r_2 c_2$ for
%$e^k=ij$, pair $\sigma$ with the term $\sigma'$ that is identical except
%it is assigned entries $r_2 c_1$ and $r_1 c_2$.
%  Since the permissible
%entries containing $e^k$ form a submatrix, the entries for $\sigma$ are both
%above the diagonal iff those for $\sigma'$ are.
%If both entries are  above the
%diagonal then $\sigma$ and $\sigma'$ both contain the product
%$x^{ek}_{ir1}y^{ek}_{jc1}x^{ek}_{ir2}y^{ek}_{jc2}$. So $\sigma$ and $\sigma'$
% have the same
%indeterminates.  They have have
%opposite sign so they
%cancel.  The argument is similar if
%the entries for $\sigma$ and $\sigma'$ are both
% below the diagonal.
%
%\bigskip
%
%The terms $\sigma$ of $\det(B(G))$ that do not fall into this case
%use an entry for an edge $e_k$ at most twice, once above and once below
%the diagonal. So $F_\sigma$ consists of copies of edges $e_k$ of
%multiplicity $\le 2$.
%
%The two remaining cases follow the theorem verbatim.
%
%Now, we show that $\F.$ is surjective.
%Let $F_1$ and $F_2$ be two $f$-factors. Observe that
%connected components of $F_1 \uplus F_2$ are Eulerian. For each
%component of $F_1 \uplus F_2$ construct an Eulerian tour. Contract these tours to obtain a directed set of tours $\sigma$.
%However, we list each self-loop twice at the beginning of $\sigma$. We will show that this tour can be associated with a
%term of $\det(B(G))$. Observe that for each vertex $v$ we have $f(v)$ outgoing edges, and $f(v)$ incoming edges.
%We associate outgoing edges from $v$ with rows corresponding to $v$, whereas incoming are associated with columns
%corresponding to $v$. We start by associating loops. The first copy of a the $k$'th loop $ii$ is
%associated with $k$'th row associated with $v$ and $f(v)-k$'th column associated with $v$, whereas the second copy is associated with
%$f(v)-k$'th row and $k$'th column. The remaining edges are associated in the order they appear
%to the next free row and column. In this way we construct a term that has a unique entry in each row,
%as well as each column. Moreover, observe that $F_1 \uplus F_2$ consists of edges of multiplicity $2$, plus
%edges of multiplicity 1 that are partitioned into even cycles. As argued previously, all such terms do not cancel with
%other terms.
%\end{proof}


==> determinant-young.tex <==
\section{Determinant formulations for general graphs}
\label{sec:determinant}
Let $G$ be a simple graph with vertices numbered from 1 to $n$.
Let $\phi=\sum_i f(i)$. We
define a skew-symmetric $\phi \times \phi$ matrix $B(G)$ representing $G$ in the following
way. A vertex $i\in V$ is associated with
$f(i)$ consecutive rows and columns of $B$, both indexed by the pairs $i,r$ for $0\le r<f(i)$.
Call a tuple $(i,r,j,c)$ representing the entry $B(G)_{i,r,j,c}$
{\it permissible} if either
\[i<j, %
\text{ or } i=j \text{ and } r<\f{f(i)/2}\le \c{f(i)/2}\le c<f(i).
\]
The set of permissible entries is denoted by $\mathbb P$.
Note that the permissible entries of $B(G)$ are all above the diagonal.
The permissible entries corresponding to a fixed edge $e$
form  a
rectangular submatrix for a nonloop $e$ and 
an $\f{f(i)/2} \times \f{f(i)/2}$ submatrix for a loop $ii$.

Using indeterminates $x^{ij}_{r}$, $y^{ij}_{c}$ we define an entry of $B(G)$ as
\begin{equation}
\label{SimpleGenMatrixEqn}
B(G)_{i,r,j,c} = % \!=\!
\begin{cases}
x^{ij}_{r} y^{ij}_{c}& %
ij\!\in\! E \text{ and } (i,r,j,c)\in \mathbb P,\\ % \text{ is permissible,}\cr
-x^{ji}_{c} y^{ji}_{r}&  %
ij\! \in\! E \text{ and } (j,c, i,r)\in \mathbb P,\\ % \text{ is permissible,}\cr
0&\text{otherwise.}
\vspace{-0.1cm}
\end{cases}
\end{equation}
Clearly $B(G)$ is skew-symmetric. Note that a loop $ii\in E$ is represented by
an $\f{f(i)/2}\times \f{f(i)/2}$ submatrix that is empty
if $f(i)=1$. This is fine since $ii$ is not in any $f$-factor.

The analysis for multigraphs is almost identical to simple graphs.
So we will concentrate on simple graphs, but also point out the extension to multigraphs.
Towards this end we extend the definition of $B(G)$ as in Section \ref{section:biparite:formulations}:
Let $\mu(e)$ denote the multiplicity of any edge $e$. The copies of $e=ij$ get
indeterminates $x^{ij,k}_{r}$, $y^{ij,k}_{c}$ ($1\le k\le \mu(e)$) and we define $B(G)$ by
\begin{equation}
\label{MultiGenMatrixEqn}
B(G)_{i,r,j,c} =
\begin{cases}
{\sum _{k=1}^{\mu(e)} x^{ij,k}_{r} y^{ij,k}_{c}}& %
\minibox{$ij\in E$  and $(i,r,j,c) \in \mathbb P$,}\vspace{3pt}
 \\\vspace{3pt} %\text{ is permissible,}\cr
-\sum _{k=1}^{\mu(e)} x^{ji,k}_{c} y^{ji,k}_{r}&  %
\minibox{$ij \in E$  and  $(j,c, i,r) \in \mathbb P$,}\\% \text{ is permissible,}\cr
0&\text{otherwise.}
\end{cases}
\end{equation}

\subsection{Review of the Pfaffian}

\def\pf{{\rm pf}}
\def\sgn{{\rm sgn}}

We will prove an analog of Theorem \ref{BipSimpleDetThm}. 
It is easiest to accomplish
 this using
the Pfaffian, so we begin by reviewing this concept.
Let $A$ be a skew-symmetric matrix 
of order $2h\times 2h$. Its Pfaffian is defined by
\[\pf(A)=\sum \sgn
\left(\begin{array}{ccccc}
1&2&\ldots&2h-1&2h\\
i_1& j_1&\ldots& i_h& j_h
\end{array}
 \right)
a_{i_1 j_1}\ldots a_{i_h j_h}.
\]
The above sum is over all partitions
of the integers $ [1..2h]$ into pairs
denoted as $\{i_1, j_1\},\ldots. \{i_h, j_h\}$.
Also \sgn\  denotes the sign of the permutation.
(It is easy to check that each term $\sigma$ in the summation is well-defined.
For example interchanging $i_1$ and $j_1$ does not change the 
partition. It flips both the sign of the permutation and 
the sign of $a_{i_1 j_1}$, so $\sigma$ is unchanged.)
The central property of the Pfaffian is \cite{lp} 
\begin{equation}
\label{PfEqn}
\det(A)=(\pf(A))^2.
\end{equation} 

Recall that the Tutte matrix $T$ for a graph $G$ is the skew-symmetric matrix
obtained from the adjacency matrix of $G$ by replacing the entry
1 for edge $ij$ by an indeterminate $t_{ij}$ if $i<j$ and by $-t_{ji}$ if
$i>j$. Clearly there is a 1-1 correspondence between perfect matchings
of $G$ and terms of $\pf(T)$. 

Recalling \eqref{PfEqn}, 
note that every pair of perfect matchings
 of $G$ get combined in the product $(\pf(T))^2$.
Let us review a proof that
no cancellations occur when all these terms are added.

Consider a term $\sigma$ of
$(\pf(T))^2$ corresponding to perfect matchings $M_1,M_2$.
(These matchings may be distinct or identical.)
The terms of 
$(\pf(T))^2$ that might cancel $\sigma$
must use exactly the same variables $t_{ij}$. In other words
they correspond to
perfect matchings $N_1,N_2 $ 
where 
\begin{equation}
\label{MNEqn}
M_1\uplus M_2=N_1\uplus N_2.
\end{equation}
$M_1\uplus M_2$ consists of the edges of 
$M_1\cap M_2$ taken twice, plus the set
$M_1\oplus M_2$. The latter  is a collection \C. of even alternating cycles.
The definition of matching shows every cycle of \C. is alternating wrt
$N_1,N_2 $. Assume that in
$(\pf(T))^2$, the first copy of $\pf(T)$ gives the matching $N_1$
and the second copy gives
$N_2$. The edges of
each cycle of $\C.$ can be partitioned
in two ways between $N_1$ and $N_2$.
So 
there are precisely $2^{|\C.|}$ matching pairs $N_1,N_2$
of $(\pf(T))^2$ that  satisfy \eqref{MNEqn}.
 
We will show there are no cancellations 
because each matching pair gives the same term of $(\pf(T))^2$.
%In other words  
More precisely we show the following:

\claim 1 {%
The pairs $N_1,N_2$ satisfying \eqref{MNEqn} collectively contribute
the quantity $s 2^{|\C.|} \Pi t_{ij}$ to $(\pf(T))^2$, where $s\in \{1,-1\}$
and the product is over the above-diagonal entries in $T$ corresponding to
$M_1 \uplus M_2$.}



\noindent
 Note the claim also implies that if we do arithmetic
over a finite field of characteristic $>2$, again there are no cancellations.

\def\bcproof #1 {\noindent{\em Proof of Claim #1.} }

\bcproof 1
Let $N$ be one of the above matchings $N_1,N_2$.
The term of $\pf(T)$
for $N$ can be written as
\[\sgn(\pi_1 \ldots \pi_k)\tau_1\ldots \tau_k.
\]
Here $k$ is the number of connected components of
$M_1\uplus M_2$ (i.e., $k =|\C.|+|M_1\cap M_2|$)
and for $1\le i\le k$,
$\pi_i$ is a permutation corresponding to the edges of $N$ in the
$i$th connected component, and $\tau_i$ is the product of the entries
in $T$ for those edges. Since the sign of a permutation is  multiplicative
the above term equals 
$\Pi_{i=1}^k \sgn(\pi_i)\tau_i$.
So the term in $(\pf(T))^2$ for the 
pair of matchings $N_1,N_2$ equals
$\Pi_{i=1}^k \sgn(\pi_i)\tau_i\cdot\sgn(\pi'_i)\tau'_i$,
where we have used
$\pi_i, \tau_i$ 
and  $\pi'_i, \tau'_i$ for 
$N_1$ and $N_2$ respectively.
This expression does not depend on choice of $N_1,N_2$
since the two halves always give the alternate edges of the component of \C.
(or the same edge of $M_1\cap M_2$ for the other components).
\ecproof

\iffalse
 plus the number
consists of the edges of 

; equivalently, 
the term for each pair has the 
same sign. Specifically the sign is $(-1)^{|\C.\cup \I.|}$,
where \I. is the set of edges $M_1\cap M_2$.
Each edge $ij$ of \I. corresponds to a transposition $(i j)$ in

Consider an even cycle of $\C.$,
$(i_1,i_2,\ldots, i_\ell)$, $\ell>2$ even.
One matching corresponds to a Pfaffian term 
containing
$\sgn\left(\begin{array}{ccccccc}
1&2&3&4&\ldots&\ell-1&\ell\\
i_1&i_2&i_3&i_4&\ldots&i_{\ell-1}&i_\ell
\end{array}\right ) 
t_{i_1i_2}t_{i_3i_4}\ldots t_{i_{\ell-1}i_\ell}$.
The other contains   
$\sgn\left(\begin{array}{ccccccc}
1&2&3&4&\ldots&\ell-1&\ell\\
i_2&i_3&i_4&i_5&\ldots&i_{\ell}&i_i
\end{array}\right )
t_{i_2i_3}t_{i_4i_5}\ldots t_{i_{\ell}i_1}$.
These permutations
differ by the product of $\ell-1$ transpositions
$(i_1 i_2)(i_1 i_3)\ldots (i_1 i_{\ell})$. So they have opposite sign.
Thus the product has sign $-1$.
\fi



We shall use one other simple property of the Pfaffian:
the relationship between two terms of $\pf(T)$
whose matchings  are identical except
that they choose alternate edges of a cycle of length 4.
Let this cycle be
$(i_1,i_2,i_3,i_4)$, and let it be component number 1 in
the notation introduces in Claim 1's proof.
The two matchings
have $\pi_1 \tau_1$ equal to
\[\left(\begin{array}{ccccccc}
1&2&3&4&5&\ldots&n\\
i_1&i_2&i_3&i_4&1&\ldots&1
\end{array}\right )   t_{i_1 i_2} t_{i_3 i_4}
\text{ and }
\left(\begin{array}{ccccccc}
1&2&3&4&5&\ldots&n\\
i_2&i_3&i_4&i_1&1&\ldots&1
\end{array}\right )   t_{i_2 i_3} t_{i_4 i_1}.
\]
(Unlike above, here the entries of $T$ needn't be above-diagonal.) The two permutations differ by the product of 3 transpositions
$(i_1 i_2)(i_1 i_3)(i_1 i_4)$. So they have opposite sign, i.e.,
the two above expressions equal
\begin{equation}
\label{SimilarPTermsEqn}
\pm  t_{i_1 i_2} t_{i_3 i_4} \text{ and } \mp t_{i_2 i_3} t_{i_4 i_1}
\end{equation}
for some consistent choice of sign.

\subsection{Analysis of {\boldmath $B(G)$}}
We return to the matrix $B(G)$ for $f$-factors.
An entry of $B(G)$ obviously corresponds to an edge of $G$, so a term of
 $\pf(B(G))$ corresponds to a multiset of edges of $G$.

\claim 2 {Each term $\sigma$ in $\pf(B(G))$ corresponds to an $f$-factor of $G$.}

\bcproof 2
The above discussion shows
that ignoring sign, 
$\sigma$ is a product of $\phi/2$ quantities
$x^{ij}_ry^{ij}_c$
corresponding to edges that form a matching on 
vertices designated by two indices
$i,r$ ($1\le i\le n$, $0\le r<f(i)$).
So
each vertex $i$ of $G$ is on exactly $f(i)$ of 
the $\phi/2$ edges selected by $\sigma$.
To show these edges form an $f$-factor of $G$ we must show
that
$\sigma$ uses each edge of $G$ at most
once. We accomplish this 
by showing that in the summation of the Pfaffian,
terms using an edge more than once
cancel in pairs.

Suppose $\sigma$ uses edges
$x^{ij}_ry^{ij}_c$ and $x^{ij}_{r'}y^{ij}_{c'}$.
Wlog assume $(i,r;j,c),(i,r';j,c')
\in \mathbb P$. $\sigma$ may have many such duplicated pairs.
Choose the duplicated pair that lexically minimizes
$(i,r,r')$. 
Pair $\sigma$ with the term $\sigma'$
having the same partition except that it replaces
$\{i,r;j,c\}$ and $\{i,r';j,c'\}$
by
$\{i,r;j,c'\}$ and $\{i,r';j,c\}$.
Note that 
permissibility of
$(i,r;j,c)$ and $(i,r';j,c')$
implies permissibility of
$(i,r;j,c')$ and $(i,r';j,c)$, even if $i=j$.
In other words $\sigma'$ is also associated with $(i,r,r')$, so the pairing is well-defined. 


Viewed as matchings, $\sigma$ and $\sigma'$ differ only by
choosing alternate edges of the length 4 cycle
$(i,r;j,c;i,r';j,c')$.
So $\sigma$ and $\sigma'$ are identical except for the expressions of
\eqref{SimilarPTermsEqn}, which in the new setting become
\[
\pm  b_{i,r;j,c}\, b_{i,r'; j,c'} \text{ and } \mp b_{j,c;i,r'} \,b_{j,c'; i,r},
\] where $b$ designates matrix $B(G)$. Substituting the
definition of $B(G)$ shows these expressions are
\[
\pm (+x^{ij}_ry^{ij}_{c}) (+x^{ij}_{r'}y^{ij}_{c'})
\text{ and }
\mp (-x^{ij}_{r'}y^{ij}_{c}) (-x^{ij}_{r}y^{ij}_{c'}).
\]
The two minus signs in the second expression follow from
permissibility of
$(i,r;j,c')$ and $(i,r';j,c)$. 
The 4 indeterminates in the 2 above expressions are collectively identical.
So we get $\sigma=-\sigma'$, i.e.,
these two terms cancel each other as desired.

This argument also applies to multigraphs $G$. Here the issue is
that only one copy of each distinct edge $ij,k$ can  used.
A term $\sigma$ with a duplicated edge, like
$x^{ij,k}_ry^{ij,k}_c$ and $x^{ij,k}_{r'}y^{ij,k}_{c'}$,
chooses the duplicated pair to lexically minimize $(i,k,r,r')$.
The rest of the argument is unchanged.
\ecproof


It is easy to see that every $f$-factor $F$ of $G$
has an uncancelled term $\sigma$ in $\pf(B(G))$: 
For each $i\in V$, order the set $\delta(i,F)$ arbitrarily.
This makes $F$ correspond to a term $\sigma$ in $\pf(B(G))$. 
Each variable $x^{ij}_r$, $y^{ij}_c$ in $\sigma$ specifies
its edge, so $\sigma$ corresponds to a unique $f$-factor $F$.
(Of course a given $F$ gives rise to many different terms.)

Let us extend this construction to an arbitrary pair of $f$-factors 
$F_1,F_2$. 
As before for each $i\in V$
and for each $F_j$ ($j=1,2$), 
number the edges of $\delta(i,F_j)$ (consecutively, starting at 1).
But now for both sets start with the edges of
$\delta(i,F_1\cap F_2)$, using the same numbering for both.
Using both these numberings together to select $\phi$ entries of $B(G)$, we a term $\sigma$ of $(\pf(B(G)))^2$. 
Each variable $x^{ij}_r$ ($y^{ij}_c$) in $\sigma$ specifies
its edge and corresponds to a unique $y_{ij}_c$ ($x^{ij}_r$).
Here we are using the fact that an edge in both $f$-factors
gives rise to a subexpression of the form $(x^{ij}_r y^{ij}_c)^2$ in $\sigma$. 

Say that  a term of   $(\pf(B(G)))^2$ is
{\em consistent} if every edge $ij$
that appears (in the superscript of an indeterminate)
has a unique  $x^{ij}_r$ and a unique $ y^{ij}_c$. 
In other words either the edge appears once as
$x^{ij}_r y^{ij}_c$ or twice as $(x^{ij}_r y^{ij}_c)^2$.
(We are disqualifying terms with an edge appearing as
$x^{ij}_r y^{ij}_c$ and also $x^{ij}_{r'} y^{ij}_{c'}$
where $r\ne r'$ or $c\ne c'$.) 
Clearly the above construction gives consistent terms.
We will show there is no cancellation 
in $(\pf(B(G)))^2$ 
involving consistent terms.
(After that we will comment on inconsistent terms.)

  


 of $G$
has an uncancelled term $\sigma$ in $\pf(B(G))$: 
For each $i\in V$, order the set $\delta(i,F)$ arbitrarily.
This makes $F$ correspond to a term $\sigma$ in $\pf(B(G))$. 
Each variable $x^{ij}_r$, $y^{ij}_c$ in $\sigma$ specifies
its edge, so $\sigma$ corresponds to a unique $f$-factor $F$.
(Of course a given $F$ gives rise to many different terms.)



\iffalse
Now
it is easy to see that \eqref{PfEqn}
gives the second part of the lemma.
But we will prove the stronger claim of surjectivity.
\fi

Next
we claim that 
the terms of $\det(B(G))=(\pf(B(G)))^2$ correspond to pairs of $f$-factors of $G$.
We prove the claim by showing that
the analysis for matchings can be applied to a {\em subset} of the terms.
After giving the proof we comment on the terms that get overlooked.





as in the case of matchings analyzed above, there is no
further cancellation when we square the Pfaffian, i.e.,
The proof follows the Tutte matrix argument:
Each term in $(\pf(B(G)))^2$ corresponds to a

Consider any pair of $f$-factors
$F_1,F_2$.
Identify terms sigma1 sigma2 in 

 that we view as matchings $FM_1, FM_2$ on vertices $i,r$. 
Another pair of $f$-factors $H_1,H_2$ involves the same
set of indeterminates exactly when $FM_1\uplus FM_2=HM_1\uplus HM_2$
and furthermore, each edge $ij$ is chosen with the same indices $r.c$
(Here we use the fact that as in the Tutte matrix,
each indeterminate $x^{ij}_r$ specifies its edge $ij$
as well as its corresponding indeterminate 
$y^{ij}_c$, and similarly for each indeterminate
$y^{ij}_c$.)
Viewing the $f$-factors as matchings on the vertices $i,r$,
the analysis for the Tutte matrix applies unchanged (more precisely the
above claim holds).




\def\FF.{\Phi_2(G)}%formerly \F._2(G) , but this is too much like \F.(G)

As in Section \ref{section:bipartite}
define $\F.$ to be the function that maps each term $\sigma$
of $\det(B(G))$
its corresponding subgraph denoted
$F_{\sigma}$.
$F_{\sigma}$ is a $2f$-factor.
Let $\FF.$ be the set
formed by taking sums of two 
(possibly equal) $f$-factors of $G$, i.e.,
\[
%\F._2(G) = \sum_{F_1, F_2: \textrm{$f$-factor of } G} F_1 \uplus F_2,
\FF.=
\{F_1 \uplus F_2: F_1, F_2\textrm{ $f$-factors of } G\} .
\]
Here $\uplus$ denotes multiset sum.
We have proved the following.


\begin{theorem}
\label{GenSimpleDetThm}
Let $G$ be a simple graph. The function $\F.$ from terms in 
$\det(B(G))$ is
a surjection onto $\FF.$. 
Consequently, $G$ has an $f$-factor if and only if $\det(B(G))\ne 0$.
\end{theorem}


Now consider multigraphs. Let $\mu(e)$ denote the multiplicity of any edge $e$. Redefine $B(G)$ as
\begin{equation}
\label{MultiGenMatrixEqn}
B(G)_{i,r,j,c} =
\begin{cases}
{\sum _{k=1}^{\mu(e)} x^{ij,k}_{r} y^{ij,k}_{c}}& %
\minibox{$ij\in E$  and $(i,r,j,c) \in \mathbb P$,}\vspace{3pt}
 \\\vspace{3pt} %\text{ is permissible,}\cr
-\sum _{k=1}^{\mu(e)} x^{ij,k}_{c} y^{ij,k}_{r}&  %
\minibox{$ij \in E$  and  $(j,c, i,r) \in \mathbb P$,}\\% \text{ is permissible,}\cr
0&\text{otherwise.}
\end{cases}
\end{equation}


The analysis is essentially identical. The proof
that a term in $\pf(B(G))$ corresponds to an $f$-factor of $G$
is unchanged -- the argument shows we cannot use more than one copy
of each distinct edge $ij,k$.
We get the following corollary.

\iffalse
As in the case of bipartite multigraphs (compare with \eqref{MultiBipartiteMatrixEqn}) we
are now representing edge $ij$ by a submatrix of rank $\mu(ij)$. Thus
Lemma~\ref{lemma-submatrix} ensures that the edge $ij$ is used no more than 
a total of $2\mu(ij)$ times.
Hence, we obtain the following corollary.
\fi


\begin{corollary}
\label{GenMultiDetThm}
Let $G$ be a multigraph. The function $\F.$ from terms in $\det(B(G))$ is
a surjection onto $\FF.$. Consequently, $G$ has an $f$-factor if and only if $\det(B(G))\ne 0$.
\end{corollary}

%\begin{proof}
%The argument closely follows those of Theorem~\ref{GenSimpleDetThm}.  We just point out the small
%differences.
%
%First, we show that the image of $\F.$ is contained in $\F._2(G)$.
%Assume that $\det(B(G))\ne 0$.  We consider three types of terms
%$\sigma$.
%
%\case{$\sigma$ uses two entries of $B(G)$ for the same edge $e_k$ of $G$,
%both above the diagonal or both below the diagonal}
%
%We pair such terms $\sigma$ so they cancel, the same way as before,
%in two steps.
%
%First associate two duplicate entries with $\sigma$: form tuples $(e_k,\min\{r_1,r_2\}$, $\max\{r_1,r_2\}$,
%$\min\{c_1,c_2\}$, $\max\{c_1,c_2\})$ to assign the edge $e_k$ in $r_1c_1$, $r_2c_2$ to $\sigma$.
%
%Now the argument follows the theorem:
%If $\sigma$ is assigned the two entries $r_1 c_1$ and $r_2 c_2$ for
%$e^k=ij$, pair $\sigma$ with the term $\sigma'$ that is identical except
%it is assigned entries $r_2 c_1$ and $r_1 c_2$.
%  Since the permissible
%entries containing $e^k$ form a submatrix, the entries for $\sigma$ are both
%above the diagonal iff those for $\sigma'$ are.
%If both entries are  above the
%diagonal then $\sigma$ and $\sigma'$ both contain the product
%$x^{ek}_{ir1}y^{ek}_{jc1}x^{ek}_{ir2}y^{ek}_{jc2}$. So $\sigma$ and $\sigma'$
% have the same
%indeterminates.  They have have
%opposite sign so they
%cancel.  The argument is similar if
%the entries for $\sigma$ and $\sigma'$ are both
% below the diagonal.
%
%\bigskip
%
%The terms $\sigma$ of $\det(B(G))$ that do not fall into this case
%use an entry for an edge $e_k$ at most twice, once above and once below
%the diagonal. So $F_\sigma$ consists of copies of edges $e_k$ of
%multiplicity $\le 2$.
%
%The two remaining cases follow the theorem verbatim.
%
%Now, we show that $\F.$ is surjective.
%Let $F_1$ and $F_2$ be two $f$-factors. Observe that
%connected components of $F_1 \uplus F_2$ are Eulerian. For each
%component of $F_1 \uplus F_2$ construct an Eulerian tour. Contract these tours to obtain a directed set of tours $\sigma$.
%However, we list each self-loop twice at the beginning of $\sigma$. We will show that this tour can be associated with a
%term of $\det(B(G))$. Observe that for each vertex $v$ we have $f(v)$ outgoing edges, and $f(v)$ incoming edges.
%We associate outgoing edges from $v$ with rows corresponding to $v$, whereas incoming are associated with columns
%corresponding to $v$. We start by associating loops. The first copy of a the $k$'th loop $ii$ is
%associated with $k$'th row associated with $v$ and $f(v)-k$'th column associated with $v$, whereas the second copy is associated with
%$f(v)-k$'th row and $k$'th column. The remaining edges are associated in the order they appear
%to the next free row and column. In this way we construct a term that has a unique entry in each row,
%as well as each column. Moreover, observe that $F_1 \uplus F_2$ consists of edges of multiplicity $2$, plus
%edges of multiplicity 1 that are partitioned into even cycles. As argued previously, all such terms do not cancel with
%other terms.
%\end{proof}


==> intro_-old.tex <==
\section{Introduction}

$b$-matching and $f$-factors are basic combinatorial notions that generalize non-bipartite matching,
min-cost network flow, and others.
This paper presents the first efficient algebraic algorithms for both weighted and unweighted $b$-matchings
and $f$-factors. Our algorithms for this broad class of problems are the most efficient algorithms known for
a subclass of instances (graphs of high density, low degree constraints
and low edge weights). We also discuss single-source all-sinks shortest paths in conservative undirected graphs.
(There is no known reduction to directed graphs.) We prove the existence of a simple  shortest-path
"tree" for this setting. We also  give efficient algorithms
-- combinatoric for sparse graphs and algebraic for dense -- to construct it.


We must first   define  $b$-matching and $f$-factors. The literature is
inconsistent but in essence we follow the classification of Schrijver \cite{Schrijver}.
For an undirected multigraph $G=(V,E)$
with a function
$f:V\to \mathbb Z_+$, an
{\em $f$-factor} is a subset of edges
wherein each vertex $v\in V$ has degree exactly $f(v)$.
For an undirected graph
$G=(V,E)$
with a function
$b:V\to \mathbb Z_+$,
a (perfect) {\em $b$-matching}
is a function $x:E \to \mathbb{Z}_+$ such that each $v\in V$ has $\sum_{w: vw\in E} x(vw) = b(v)$.
The fact that $b$-matchings have an unlimited number of copies of each edge
makes them decidedly simpler. For instance
$b$-matchings have essentially the same blossom structure
(and linear programming dual variables)
as
ordinary matching \cite[Ch.31]{Schrijver}. Similarly our algorithm
for weighted $b$-matching is almost identical to its specialization to ordinary matching ($b\equiv 1$).
In contrast the blossoms and dual variables for weighted $f$-factors are more involved \cite[Ch.32]{Schrijver}
 and our algorithm
is more intricate.
Thus our terminology reflects the difference in complexity of the two notions.%
\footnote{Another version of $b$-matching considers $b(v)$ as an upper bound on the desired degree of $v$.
This easily reduces to weighted perfect $b$-matching by taking 2 copies of $G$ joined by
zero-weight edges.
On the other hand a {\em capacitated $b$-matching}
is defined by giving an upper bound $u(e)$ to each value $x(e)$.
The simplicity of
the uncapacitated case is lost, and we are back to $f$-factors.}

The paper begins with unweighted $f$-factors, i.e., we wish to find an $f$-factor
or show none exists. Let $\phi=f(V)$ (or $b(V)$).
We extend the Tutte matrix from matching to $f$-factors,
i.e., we present a $\phi \times \phi $ matrix that is
symbolically nonsingular iff the graph has an $f$-factor.
Such a matrix can be derived by applying the Tutte matrix to an enlarged version of the given graph,
or by specializing Lov\'asz's matrix
for matroid parity \cite{l}. But neither approach is compact enough to achieve our time bounds.%
\footnote{The Tutte matrix becomes too large, $m\times m$. Lov\'asz's matrix
is $\phi \times \phi$ but can involve
integers that are too large,  size $n^n$ or more. Our matrix only involves integers $\pm 1$.}
Then we reuse the elimination framework for maximum cardinality matching, due to
Mucha and Sankowski~\cite{ms04} and Harvey~\cite{Harvey06}. This allows us to find an $f$-factor in $O(\phi^{\omega})$ randomized time.%
\footnote{$O(n^{\omega})$ is the time needed for a straight-line program to multiply two $n\times n$ matrices; the best-known bound on $\omega$ is $<2.3727$~\cite{Williams}.} For dense graphs
and small degree-constraints this improves the best-known time bound of $O(\sqrt{\phi} m)$ \cite{hal83},
although the latter is deterministic.

\iffalse
The development of our algorithms would be impossible
without the recent advance in development of the combinatoric interpretation of dual variables for perfect matchings~\cite{CGSa,G}
as well as for $b$-matchings and $f$-factors~\cite{G}. This interpretation was the most crucial part that led to the first
$\tilde{O}(Wn^{\omega})$ time algorithm for finding minimum weight perfect matchings in graphs~\cite{CGSa}. It allows to relate
the dual problem to the perturbed primal problem and opens the way for the efficient computation of the dual variables
(for definition of perturbed problems we refer to Section~\ref{BackgroundSec}).
Here, we show how to turn this interpretation into efficient solutions for $f$-matching and $f$-factor problems
obtaining $O(W\phi^{\omega})$ randomized time algorithms. This result
improves upon previously known algorithms for dense graphs -- please see Table~1 and Table~2.
Our algorithms can be easily turned into Las Vegas algorithms, since we can check the optimality by using
dual variables.
%Our weighted algorithms imply $O(\phi^{\omega})$ time algorithm for computing maximum size $b$-matching as well.
\fi

\begin{center}
    {
    \noindent
      \begin{tabular}{|p{5cm}|p{4.0cm}|} \hline
        Time & Author \\ \hline
        $O(n^2 B)$  & Pulleyblank (1973) \cite{Pulleyblank}\\ \hline
        $O(n^2 m \log B)$ & Marsh (1979) \cite{Marsh}\\ \hline
        $O(m^2 \log n \log B)$ & Gabow (1983) \cite{hal83}\\ \hline
        $O(n^2 m + n \log B(m+n\log n))$ & Anstee (1987) \cite{anstee}\\ \hline
        $O(n^2 \log n(m+n\log n))$ & Anstee (1987) \cite{anstee}\\ \hline
        $\tilde{O}(W\phi^{\omega})$ & this paper\\ \hline
      \end{tabular}

      \vspace{0.2cm}
      {\bf Table 1:} Time bounds for maximum $b$-matching. $B$ denotes $\max_v b(v)$.
    }
\end{center}

\begin{center}
    {
    \noindent
      \begin{tabular}{|p{3.1cm}|p{4.8cm}|} \hline
        Complexity & Author \\ \hline
        $O(\phi n^3)$ & Urquhart (1965) \cite{urquhart} \\ \hline
        %$O(\phi m \log n)$ & Gabow (1983) \cite{hal83}\\ \hline
        %$O(\phi n^2)$ & Gabow (1983) \cite{hal83}\\ \hline
%$O(\phi(m+n \log n))$ & Gabow (1990) \cite{gabow-90}  \\ \hline
$O(\phi(m+n \log n))$ &
Gabow (1983$+$1990) \cite{hal83, gabow-90} \\ \hline
        $\tilde{O}(W\phi^{\omega})$ & this paper\\ \hline
      \end{tabular}

      \vspace{0.2cm}
      {{\bf Table 2:} Time bounds for maximum weight $f$-factors on simple graphs.}
}
\end{center}

We turn to the more difficult weighted version of the problem. Here every edge has a numeric
weight; for complexity results we assume  weights are  integers of magnitude
$\le W$.
We seek a {\em maximum
$f$-factor}, i.e., an $f$-factor with the greatest possible total weight.
Efficient algebraic algorithms
have been given for maximum matching ($f\equiv 1$) in time $\tilde{O}(W n^\omega)$,
first for bipartite graphs \cite{Sankowski09} and recently for general graphs \cite{CGSa}.\footnote{The $\tilde{O}$ notation ignores factors of
$\log (n\phi W)$.}% and $\log W$.}

The usual approach to generalized matching problems is by problem reduction.
For instance
in \cite{Schrijver}, Ch.31
proves the properties of the $b$-matching linear program and polytope
by reducing to ordinary matching via vertex splitting;
then Ch.32 reduces $f$-factors (capacitated $b$-matching) to $b$-matching.
Efficient algorithms also use vertex splitting \cite{hal83}
or
reduction
to  the bipartite case (plus by further processing) \cite{anstee}.
But reductions may obscure some structure.
To avoid this our algorithms use a direct approach, and we get the following rewards.
For $b$-matching, as mentioned, the similarity of blossoms to
ordinary matching blossoms leads to an algorithm that is no more involved than
ordinary matching.
For undirected shortest paths we get a simple definition of a generalized shortest-path tree.
(Again such a definition may have been overlooked due to reliance on reductions, see below.)
For $f$-factors we get a detailed understanding of the more complicated versions of
the structures that first emerge in $b$-matchings
(2-edge connected components giving the cyclic part of blossoms -- see Section \ref{VBSec})
and in shortest paths (bridges giving the incident edges of blossoms --
these correspond to
the (ungeneralized) shortest-path tree -- see Section \ref{IBSec}).

All three of our non-bipartite algorithms are implementations of
the "shrinking procedure" given in \cite{G} (a variant is the basis of the weighted matching
algorithm of \cite{CGSa}).
This procedure gives a direct way to find the optimum blossoms for a weighted $f$-factor --
simply put,
each blossom is (a subgraph of) a maximum weight "$2f$-unifactor" (a type of $2f$-factor) in
the graph with (the cyclic part of) all heavier blossoms contracted
(see \cite{G} or Section \ref{BackgroundSec}). Note that the classic weighted matching algorithm of Edmonds
\cite{e} finds the optimum blossoms, but only after  forming and discarding
various other blossoms. So this approach does not provide a direct definition of the optimum blossoms.

The first step of our algorithms use our generalized Tutte matrix to find
the optimum dual variables of the vertices.  Then we execute  the shrinking procedure to
get the blossoms, their duals, and a "weighted blossom tree" that gives the structure of the optimum $f$-factor.
(This step is combinatoric. It is based on the detailed structure of 
$2f$-unifactors that we derive.)
The last step finds the desired $f$-factor  using
a top-down traversal of
the weighted blossom tree: At each node
we find an $f$-factor of a corresponding graph, using our algorithm for unweighted $f$-factors.
In summary our algorithms (like \cite{CGSa} for ordinary matching) can be viewed as a (combinatoric) reduction of the weighted
$f$-factor problem into two subproblems: finding the optimum dual variables of the vertices,
and finding an unweighted $f$-factor.

To facilitate understanding of the general $f$-factor algorithm we begin by presenting its specialization to
two subcases. First $b$-matching.
The blossoms, and hence the $2b$-unifactors, differ little from ordinary graph
matching. As a result our development for weighted $b$-matching  is essentially  identical
the special case of ordinary matching, in terms of both the underlying combinatorics and the algorithmic details.
When specialized to ordinary matching our algorithm provides a simple alternative to \cite{CGSa}. In fact an advantage
is that our algorithm is Las Vegas -- the dual variables allow us to check if the $b$-matching is truly optimum.
(Our approach to weighted matching/$b$-matching differs from \cite{CGSa} -- at the highest level,
we work with critical graphs while \cite{CGSa} works with perfect graphs.)

Next we discuss shortest paths in undirected graphs with a conservative weight function --
negative edges are allowed but not negative cycles. The obvious reduction to a directed graph
(replace undirected edge $uv$ by directed edges $uv,vu$) introduces negative cycles, and it is
unclear how to handle this problem by the usual shortest-path techniques.

We consider the
single-source all-sinks version of the problem.
Again, this problem is often solved by reduction, first to the single-source single-sink
version and then to perfect matching, using either T-joins
\cite[pp.485--486]{Schrijver}
or vertex-splitting
\cite[p.487]{Schrijver}.
A path can be viewed as a type of 2-factor.
(For instance an $ab$-path is an $f$-factor
if we enlarge $G$ with a loop at every vertex $v\in V$
and set $f(v)=2$ for $v\in V-\{a,b\}$, $f(a)=f(b)=1$.)
This enables us to
solve the all-sinks version directly. Examining the
blossom structure
enables us to
define a generalized shortest-path tree that, like the standard shortest-path tree for directed graphs,  specifies a shortest path to every vertex from a chosen source.
It is a combination of the standard shortest-path tree and
the blossom tree. We give a complete derivation of the existence of this shortest-path structure, as well
as an algebraic algorithm to construct it in time $\tilde{O}(Wn^\omega)$. We also construct the structure
with combinatoric algorithms, in time
$O(n(m+n\log n))$ or $O(\sqrt{n \alpha(m,n)\log n}\ m \log (nW))$. These bounds are all
within logarithmic factors of the best-known bounds for constructing the directed shortest-path tree ~\cite[Ch.~8]{Schrijver}, \cite{YusterZ05,Sankowski05}.


\iffalse
Additionally, we give an improved algorithms that constructs the shortest path structure. We essentially argue that instead of calling O(n) times perfect matching subroutine, a single call to it is enough. This allows us to give  $\tilde{O}(Wn^{\omega})$ time algebraic algorithm. Similarly, we can use algorithm of Gabow~\cite{gabow-90} to obtain an $O(n(m+n\log n))$ time algorithm for computing shortest path structure, and an $O(\sqrt{n \alpha(m,n)\log n}\ m \log (nW))$ time algorithm by using results of Gabow and Tarjan~\cite{gt91}. Hence, our time bounds up to logarithmic factors match the fastest algorithms known for directed case~\cite[Ch.~8]{Schrijver} and~\cite{YusterZ05,Sankowski05}).
\fi




Although the
shortest-path problem is classic, our definition of this structure appears to be new.
Most notably, Seb\"o has characterized the structure of single-source shortest paths in undirected graphs,
first for
graphs with $\pm 1$ edge weights \cite{Sebo} and then extending  to general weights by reduction \cite{sebo2}.  Equation (4.2) of \cite{Sebo} (for $\pm 1$-weights, plus its version achieved by reduction
 for arbitrary weights)
 characterizes the shortest paths from a fixed
source
in terms of  how they enter and leave "level sets"
determined by the distance function. \cite{Sebo} also shows that the distances from the source can be computed using $O(n)$ perfect matching computations. Our structure differs from
 \cite{Sebo,sebo2}: it does not give a necessary and sufficient condition to be a shortest path, but it
gives an exact specification of a specific set
of shortest paths that are simply related to one another (as in the standard shortest-path tree). Note that one
can give an alternative proof of the existence of our structure  by starting from the results of \cite{Sebo,sebo2}.


The general algorithm for maximum $f$-factors is the most difficult part of the paper.
It involves a detailed study of the properties of blossoms. A simple example of how
these blossoms differ from ordinary matching is that the hallmark of Edmonds' blossom
algorithm -- "blossoms shrink" -- is not quite true. In other words for ordinary matching
a blossom can be contracted and it becomes just an ordinary vertex. For $f$-factors we can contract
the "cycle" part of the blossom, but its incident edges remain in the graph and must be treated differently from
ordinary edges (see Section \ref{IBSec}).
Our discussion of shortest paths introduces this difficulty in
the simplest case -- here a blossom has exactly 1 incident edge (as opposed to an arbitrary number).
Even ignoring this issue, another difficulty is that there are three types of edges that behave differently
(see \cite{G}, or Lemmas \ref{UnifactorLemma} and \ref{NUnifactorCor}) and the type of an edge is
unknown to the algorithm! Again the three types are seen to arise naturally in shortest paths.
Our contribution is to develop the combinatoric properties of these edges and blossoms
so the shrinking procedure can be executed efficiently, given only the information provided by the
Tutte matrix in our algebraic algorithm.



While non-bipartite graphs present the greatest technical challenge,
we also achieve some best-known time bounds for
two bipartite problems, maximum network flow
and min-cost network flow.
Bipartite $f$-factors generalize network flow: max-flow 
(min-cost max-flow)
is a special case of
unweighted (weighted) bipartite $f$-factors, respectively~e.g.~\cite{gabow-tarjan-89}.
The question of
an efficient algebraic max-flow algorithm has confronted the community for
some time. The only advance is the algorithm of Cheung et.~al.~\cite{cheung}, which checks
whether $d$ units of flow can be sent across a unit-capacity network in $O(d^{\omega-1}m)$ time. We 
consider
 networks with integral vertex and edge
capacities bounded by $D$.
We find a max-flow in time
$\tilde{O}((Dn)^{\omega})$ time 
and a
min-cost max-flow 
in $\tilde{O}(W(Dn)^{\omega})$ time.
%(by~\cite{gabow-tarjan-89} $D$ translates to $f$-values).
The latter algorithm handles convex edge cost functions 
(with integral break-points)
in the same
time bound.
The max-flow problem has a rich history (see e.g.~\cite[Chs.~10, 12]{Schrijver})
and our time bounds are the best-known for
dense graphs with moderately high vertex capacities. 
Specifically, previous algorithms for vertex-capacitated max-flow in dense networks (i.e., $m=\Theta(n^2)$) 
use $O(n^3/\log n)$ time~\cite{Cheriyan90} or $O(n^{8/3}\log D)$ time~\cite{Goldberg98}. 
Previous algorithms for dense graph
min-cost max-flow use $O(n^3 \log D )$ time~\cite{edmonds-karp-72} or $O(n^3\log n)$ time~\cite{Orlin88}.
Previous algorithms for
minimum convex-cost max-flow 
use $O(D n^3\log D)$ time 
(by simple reduction to min-cost max-flow)
or $O(n^4\log D)$ time~\cite{Ahuja93}.

In summary the novel aspects of this paper are:

$\bullet$
new time bounds for the fundamental problems of $b$-matching, undirected single-source shortest paths, and $f$-factors;

$\bullet$
extension of the Tutte matrix for matching to $f$-factors;

$\bullet$
definition of the shortest-path structure for undirected graphs, plus algebraic and combinatorial
algorithms to construct it;

$\bullet$
an algebraic algorithm for $b$-matching that is no more involved than ordinary matching;

$\bullet$
an algebraic algorithm for $f$-factors based on new combinatorial properties of blossoms,
which are qualitatively different from matching blossoms;

$\bullet$
new time bounds for vertex-capacitated max-flow, min-cost max-flow and minimum convex-cost max-flow on dense graphs.

\paragraph*{Organization of the paper}
The next two sections define our terminology and review the algebraic tools that we use.

Section~\ref{section:bipartite} gives an overview of the entire paper, by discussing
the special case of bipartite $f$-factors. 
(The reader should bear in mind that the non-bipartite case
is the highlight of this paper. It is technically much more demanding.)
In detail, Section~\ref{section:bipartite}  starts with an $O(\phi^{\omega})$ time algorithm
for unweighted bipartite $f$-factors. This requires our generalized Tutte matrix 
(Section~\ref{section:biparite:formulations}; 
Section~\ref{sec:determinant}
extends this to non-bipartite graphs)
plus the
algorithmic details (Section~\ref{section:biparite:algorithms};
Section~\ref{sec:algorithms} generalizes these details to non-bipartite graphs). 
Section~\ref{section:weighted-bipartite}
gives the algorithm for weighted bipartite $f$-factors. 
Flows are discussed in Section~\ref{FlowSec}.

As mentioned above the algorithms for general graphs
have three steps:

\i find the weights of factors of perturbed graphs;

\ii use the weights to construct a blossom forest;

\iii use an unweighted algorithm to extract an  optimal solution from the blossom forest.

\noindent
These steps are implemented in different sections, depending on the problem of interest.
Specifically for
{$b$}-matching,  \i is in Section~\ref{sec:weights}, \ii and \iii are in Section~\ref{GeneralbMatchingSec},
and
the unweighted algorithm of \iii is in Section~\ref{sec:algorithms}.
For shortest paths,
the algebraic algorithm for \i is in Section~\ref{sec:weights} and
the combinatoric algorithm is in Section~\ref{SPcombinatoric}.
\ii is in Section~\ref{fFactorSec} and
\iii is in Section~\ref{SPAlgSec}.
For {$f$}-factors, \i is in Section~\ref{sec:weights}, \ii and \iii are in Section~\ref{fFactorSec},
with the unweighted algorithm of \iii in Section~\ref{sec:algorithms}.


The most involved part of the paper is the construction of blossom forest for $f$-factors in Section~\ref{fFactorSec}.
This section is preceded by two sections that introduce our combinatoric ideas in simpler settings:
Section \ref{GeneralbMatchingSec} gives the combinatoric portion of our weighted $b$-matching algorithm. Section \ref{SPSec} proves the existence of our shortest-path structure.
Section~\ref{BackgroundSec} reviews fundamental background material on $f$-factors
(illustrating it by  shortest-paths).
After the combinatoric algorithm for weighted $f$-factors in Section~\ref{fFactorSec},
Section \ref{SPAlgSec} gives the   algorithm to construct the shortest-path structure,
and Section \ref{SPcombinatoric} gives the combinatorial  algorithms for shortest-path weights.
Sections~\ref{sec:determinant}--\ref{sec:algorithms}
show how to find unweighted $f$-factors in general graphs.
Section~\ref{sec:weights} shows how to compute the weights of perturbations of $f$-factors.
Finally Section \ref{ConclusionSec} concludes by posing several new open problems.




Given the length of this submission, we remark that various portions 
can be read independently.
Section~\ref{section:bipartite} gives the whole development in the bipartite case.
Section~\ref{GeneralbMatchingSec} gives the  combinatoric part of the
$b$-matching algorithm starting from first principles.
Section~\ref{SPSec} derives the shortest-path structure from first principles, entirely in the language
of shortest paths rather than matching. The related material in Section~\ref{SPAlgSec} is itself
independent, given the definition of the shortest-path structure (Section~\ref{SPDefnSec}).
Alternatively Sections~\ref{GeneralbMatchingSec}--\ref{SPSec} can be skipped to go directly
to the combinatoric part of the $f$-factor algorithm (Sections~\ref{BackgroundSec}--\ref{fFactorSec}). 




==> response.tex <==
Dear Hal,

the problem is not that the set of pairs is wrongly defined. As far as I understand everything the determinant indeed contains terms that correspond 
to pairs of f-factors. The problem is in this case in the proof. 

\case {$F_\sigma$ consists of edges of multiplicity $\le 2$, and
contains an odd cycle of edges of multiplicity 1}

There is a difference between cycles of $F_\sigma$ and cycles of the permutation used to obtain $\sigma$. 
We write: Associate $\sigma$ with the ordered pair $(i,j)$ where $i\le j$, edge
$ij$ belongs to an odd cycle $C$ of $\sigma$, and $(i,j)$ is lexically
minimum.  Pair $\sigma$ with the term $\sigma'$ that is identical to
$\sigma$ except $C$ has edges in opposite
orientation from $\sigma$. This might be impossible when the cycle $C$ actually belongs
to a cycle of the permutation witch is longer then $C$. In such a case you cannot partially
reverse the orientation of the cycle of the permutation. 

In the case of the graph containing the two triangles. We have following terms 
in the determinant:
- two terms corresponding two f-factors with doubled multiplicity of edges,
- four terms corresponding to traversal of the two triangles in different directions
- four pairs of terms corresponding to cycles of length 6 that pass through the vertex "a" twice. 

In these length 6 cycles one cannot reverse the directions of the triangles. The problem is that 
these triangles end in different rows and columns of the matrix. They end in the same vertex a, but 
it has 2 rows and 2 columns now. 

Bests,
Piotr







==> shtstpthconstr.tex <==
\section{Construction of the shortest-path structure}
\label{SPSecconstr}
The last two lemmas show how to construct the first node
of the gsp-tree. We
construct the remaining nodes by iterating the procedure.
This sections first shows how to construct the gsp-tree; then it
completes the gsp-structure by constructing $z$.

For the gsp-tree we first state the algorithm
and then prove its correctness.
{\em Shrinking a p-cycle}  means
contracting its cycle $C$; $C$ is the {\em shrunken cycle}.
Let $\o G$ be a graph formed by starting with $G$ and repeatedly
shrinking a p-cycle. (So the collection of
shrunken cycles forms a laminar family.)
We treat $\o G$ as a multigraph that contains parallel edges
but not loops. It is convenient to refer to vertices and
edges of $\o G$ by indicating the corresponding objects in $G$.
So let
$\o E(G)$ denote the set of edges of $G$ that correspond to (nonloop)
edges in $\o G$.
Thus writing
$xy\in \o E(G)$
implies
$x,y\in V(G)$. We do not distinguish between
$xy$ and its image in $\o G$.
Similarly,
writing $C,cc'$
for a shrunken p-cycle implies $cc'\in \o E(G)$,
and a $vt$-path in $\o G$ has $v\in V(G)$ and its first edge incident to $v$.
An overline denotes quantities in $\o G$, e.g., $\o w$, $\o \zeta$.
%Finally, for uniformity  we will view every vertex of $\o G$ as a set
%of vertices of $G$. Thus it makes sense to speak of a vertex of $G$ belonging
%to vertex $v$ of $\o G$, even if $v$ is not a contracted set.


The following algorithm  constructs the
gsp-tree \T.. We assume the shortest paths $P_x$ are known.
(The function $z$ is constructed below.)

\bigskip

Initialize
 $\o G$ (the current graph) to the graph
$(V,E_\ell(G))$, and
\T. to contain each vertex of $G$ as a singleton subtree.
Then repeat the following step
until %the only cycles in $\o G$ are loop nodes:
$\o G$ is acyclic:

\bigskip

{\narrower

{\parindent=0pt

Let $C,cc'$ be the p-cycle of weight $\zeta^*(\o G)$ given by Lemma
\ref{sp2.2}.  Shrink $C$ in $\o G$. %If $C$ is a loop,
Set $e(C)=cc'$. Unless $C$ is a loop,
 create a
node in \T. whose children correspond to the vertices of $C$.

}}

\bigskip


\noindent
When the loop halts create a root
node of \T. whose children correspond to the vertices of
the final graph $\o G$.%
\footnote{In contrast with the general definition,
our assumption that $t$ is on a unique edge
ensures the root of \T. is always a tree node.}

\bigskip

To complete the description of this algorithm
we must specify the weight function $\o w$ for $\o G$.
Let $\C.$ be the collection of maximal shrunken cycles that
formed $\o G$.
An edge $cc'\in \o E(G)$ may be associated
with two cycles of \C., one at each end.
For a p-cycle $C,cc'$ in \C., as in
Definition \ref{SPTreeDfn}
$V(C)$ denotes the set of vertices of $G$ that belong to
$C$ or a contracted vertex of $C$ .
$V(\C.)$ is the union of all the $V(C)$ sets.
For $C,c\in \C.$ and $x\in V(C)$,  $C_x\con E(G)$ denotes
%$xc$-subpath of $P_x$.
%(Property P2 below will show $c$ is actually in $P_x$.)
the minimum-weight $xc$-path contained in $\gamma(C,G)$.
%($C_x$ is defined by the contractions that form $C$.)

Let $G$ denote the given graph, and
let
%$\omega=2\sum\set{|w(e)|}{e\in E}$.
\[\omega=2|w|(E).\]
The weight  of an edge $e=xy\in \o E(G)$ in $\o G$ is defined to be
$\o w(e)=w(e)+\Delta(e,x)+\Delta(e,y)$, where
\[\Delta(e,x)=\begin{cases}
0&x \notin V(\C.)\\
-2\omega&\text{\C. contains p-cycle  }C,e \text{ with } x\in V(C)\\
2\omega+w(C_x)&\text{\C. contains p-cycle  }C,cc' \text{ with }x\in V(C), cc'\ne e.
\end{cases}
\]

We will use a variant
of the ``respects'' relation.
Let $\o S$ be a cycle or path in $\o G$. Let
$C,cc'$ be a p-cycle of \C., and  $\o C$ the contracted vertex
for $C$ in $\o G$.
\iffalse
%that is a cycle or a $vt$-path. Here we allow $v$ to be a vertex of $G$,
%and for $v\in V(\C.)$ a $vt$-path begins at the image of $v$.
\fi
$\o S$ {\em respects} $\o C$  if
$\o S\cap \delta(\o C)$ is either empty
or consists of $cc'$ plus $\le 1$ other edge.
This definition corresponds to the previous definition if we view $\o C$
as a p-cycle whose cycle is  a loop $\o C\,\o C$.
More importantly we shall use this fact:
If a path $P$ respects $C,cc'$ and $\o G$ is derived from $G$
by contracting $C$ to a vertex $\o C$, then the image of
$P$ in $\o G$ respects $\o C$.
Also,
for any $C,cc'$ in $\o{\C.}$,
 if the image of a  shortest path $P_u$
respects $\o C$ and contains $\o C$ internally,
then $P_u$ traverses $C$ along the path $C_x$ that joins
the 2 edges of $P_x\cap \delta(C)$.
This follows from the optimality of $P_u$.



$\o S$ {\em respects} $\o {\C.}$  if it respects each $\o C\in \C.$.
\iffalse
call the subgraph $S$ of $G$ We require $S$ to be a $vt$-path if $\o
S$ is.  We say this subgraph $S$ is
\fi
When $\o S$ respects $\o {\C.}$,
the {\em preimage} of $\o S$ is the subgraph
$S$ of $G$ that completes $\o S$ with minimum weight, i.e.,
$S$
consists of the edges of $\o S$
plus,
for each p-cycle $\o C$  on 2 edges of $\o S$,
the minimum-weight path $C_x$ in $C$ that joins
the 2 edges.
This preimage
is unique.
(Any $C,cc'$ of \C. that is on 2 edges of $\o S$ is on
$cc'$ and another edge that determines the vertex $x$
in the definition of the preimage. Note
that
if $\o S$ is a $vt$-path that respects $\o {\C.}$ and $v\in V(\C.)$
then $v=c$ for some p-cycle $C,cc'$ of \C.; so in this case
the preimage of $\o S$
does not contain any edges
of $C$.)


\iffalse
and
with $x\notin V(\o C.)$ or $x=c$ for some
 then $P_x$ is the preimage.
\fi

Lemma \ref{spContractLemma} below shows
the following properties always hold.

\bigskip

{\parindent=0pt

P1:  $\o G$ is conservative.

%P2: For any vertex $x\in V(G)$ with image $\o x$ in $\o G$, $P_{\o x}$
%is the image of $P_x$.  In fact


P2: For any vertex $x\notin V(\C.)$, $P_x$ is the
preimage of $P_{\o x}$.  For any p-cycle $C,cc'\in \C.$,
$P_c$ is the
preimage of $P_{\o C}$, both of which start with edge $cc'$.
For any other $x\in V(C)$, the image of $P_x$ in $\o G$ is $P_{\o C}$.
}

\iffalse
P3: Let $C,cc'$ be a nonloop  p-cycle of some iteration, with children $B_i,
i=1,\ldots, k$ in \T..  For any $i$, $\o E(P_{\o B_i})$ is one of the
$\o B_i\,t$-paths in the p-cycle.
\fi



\begin{lemma}
Assuming P1--P2 always hold, \T. is a valid
gsp-tree for $G$.
\end{lemma}

\begin{proof}
First observe that every vertex $x\in V(G)$ gets
assigned a  value $e(x)$.
This holds as long as some  iteration chooses $xx$ as the minimum weight
p-cycle. So for the purpose of
contradiction, suppose
an iteration contracts a p-cycle $C$
where  $x\in C$ but
the loop $xx$ has not been contracted.
Since $xx\notin P_x\oplus P_x=\emptyset$,
$xx$ is considered
in the definition of $E^*$. So we get the desired contradiction
by proving
%This makes \eqref{xxEqn} a contradiction.
\begin{equation}
\label{xxEqn}
\zeta(xx)=    w(xx)+2w(P_x)<\zeta^*.
\end{equation}
Lemma \ref{sp2.2}\iii shows
$2w(P_x)\le \zeta^*$ (in any iteration).
We can assume the perturbation of $w$
gives every subgraph of $2G$  a distinct weight.
Thus $2w(P_x)<\zeta^*$.
Furthermore we can assume the perturbation enforces a lexical ordering
of the edges. Since
the loop $xx$
is ordered after any edge of $G$, it cannot reverse
this inequality, i.e., \eqref{xxEqn} holds.

The algorithm sets $e(C)$ correctly for
each node $C$ of \T., by definition.
Recall
the path $p(v,N)$ from \eqref{PvFormEqn}.
It is easy to see the lemma amounts to proving that
for
any interior node $C$ of \T. and any vertex $x\in V(C)$, the edges of
$E(P_x)\cap \gamma(C)$ correspond to $p(x,C)$ as defined in \eqref{PvFormEqn}.
Let p-cycle $B,bb'$ be the child of $C$ with $x\in B$.
($B$  is a loop when the child of $C$ is a leaf of \T..)
We consider two similar cases for node $C$.

{\def\gm.{$\o G$}
Suppose  $C,cc'$ is a cycle node of \T..
Let \gm.  be the graph immediately before $C$ is contracted.
P2 in \gm. shows
$P_b$ is the preimage of $P_{\o B}$.
It also shows
$P_{\o B}$ starts with $bb'$.
Lemma \ref{sp2.2}\ii shows $P_{\o B} $ is one of the $\o
B\, t$-paths in the p-cycle.
We have already observed that $C$ and its children have
the correct $e$-values. Thus
\T. specifies  the desired path $p(b,C)$ as defined in  \eqref{PvFormEqn}.
This extends to any $x\in V(B)$ by the last assertion of P2.
}


%  Using the notation of
%P3, suppose $x\in V(B_i)$ for p-cycle $B_i,b_ib'_i$ (possibly a loop).


The remaining case is for the root node \V. of \T., with \V.
 a tree node. In the final acyclic graph,
%let the image of $x$ be the contracted cycle $B,bb'$.
P2 shows $P_b$ is the preimage of $P_{\o B}$.
Thus \T. specifies the desired path $p(b,\V.)$.
As before
this extends to any vertex $x\in V(B)$.
\xecproof
\end{proof}


We complete the gsp-structure by specifying $z$.  For each node $N$ of
\T. let $\zeta_N$ be the weight $\zeta^*(\o G)$ of its corresponding
p-cycle.  For a leaf $x$ the corresponding p-cycle is the loop $xx$;
for the root \V. of \T., which is a tree node, the corresponding
p-cycle is the last p-cycle to get shrunk. Let $p$ be the parent
function in \T..  For each node $N$ define

\[
z(N)=
\begin{cases}
\zeta_N&N=\V.\\
\zeta_N-\zeta_{p(N)}&N\ne \V.\\
\end{cases}
\]


Lemma \ref{spContractLemma} shows this additional property always holds:

\bigskip

{\parindent=0pt

P3:  For any $uv\in \o E(G)$,
\[
\o\zeta(uv)=\begin{cases}
\zeta(uv)&uv \notin P_u\oplus P_v\\
\zeta(uv)&uv \in P_u-P_v, u\notin V(\C.)\\
\zeta(uv)-4\omega&uv \in P_u-P_v, u\in V(\C.).
\end{cases}
\]
}

\noindent
The notation in P3 is unambiguous since
$uv\in P_u$ iff $uv\in P_{\o u}$ by P2.

\begin{lemma}
Assuming P1--P3 always hold, \T. with the above function  $z$ is a
gsp-structure for $G$.
\end{lemma}

\begin{proof}
 The definition of $z$ clearly implies
that for any node $N$ of \T.,
the $z$-values of all the ancestors of $N$ (including $N$)
sum to $\zeta_N$. We claim $\zeta^*(\o G)$ increases every iteration.
The claim implies that
for every $N\ne \V.$,
$z(N)=\zeta_N-\zeta_{p(N)}\le 0$, i.e., $z(N)$ is nonpositive as desired.
To prove the claim note that
for a fixed edge $uv$,
$uv$ belongs to $P_u\oplus P_v$
in one iteration iff it does in the next iteration,
as long as it is not contracted (by P2).
Hence
the only change in $E^*$ from one iteration to the next is that
contracted edges leave $E^*$. P3 shows the edges in $E^*$ retain their original
$\zeta$-values. Thus $\zeta^*(\o G)$ never decreases.

To complete the proof we must show
\eqref{DomEqn} for every $uv\in E_\ell(G)$, with equality for
$e(N)$ edges and other edges of subgraphs $E(N)$.
Consider two cases.

\case {$uv \notin P_u\cap P_v$}
By definition
\[d(u)+d(v)+w(uv)=\zeta(uv).\]
Let $N$ be the deepest node of \T. that covers $uv$.
Observe that
\[
\zeta(uv) \ge \zeta_N,
\]
with equality holding if $uv\in E(N)\cup e(N)$.
In proof,
if $uv\notin P_u\cup P_v$ this follows from
$uv\in E^*$.
If  $uv\in P_u- P_v$,
then Lemma \ref{SimpleLemma} shows $uv=e(u)$.
So the loop $uu$ covers $uv$, $N=\{u\}$,
and equality holds.
Since the sum of the right-hand side of \eqref{DomEqn} equals $\zeta_N$,
combining the two displayed relations gives the desired conclusion
for  \eqref{DomEqn}.

\case {$uv \in P_u\cap P_v$}
By definition
\[d(u)+d(v)-w(uv)=\zeta(uv).\]
$uv$ is covered by the nodes of \T. that are ancestors
of $u$ or $v$. The ancestors of $u$ have $z$-values summing
to $\zeta(uu)=2d(u)$ and similarly for $v$.
 Let node $A$ be the least common ancestor
of $u$ and $v$ in \T..
Since $uv$ is in the cycle of node $A$, $\zeta_A =\zeta(uv)= d(u)+d(v)-w(uv)$
(by definition of $\zeta$).
The sum of the right-hand side of \eqref{DomEqn} equals
\[\zeta_u +
\zeta_v -\zeta_A = 2d(u)+2d(v)-(d(u)+d(v)-w(uv))=
d(u)+d(v)+w(uv)\]
as desired.
\end{proof}

The development is completed by establishing P1--P3:

\begin{lemma}
\label{spContractLemma}
P1--P3 hold in every iteration.
%In each iteration the current graph $\o G$ satisfies P1--P2.
\end{lemma}

\begin{proof}
Consider two edges
$e_i=x_iy_i \in \o E(G)$, $i=1,2$,
where both $x_i$ have the same image in $\o G$.
If $x_i\notin V(\C.)$ then
\begin{equation}
\label{DelVEqn}
\Delta(e_1,x_1)+\Delta(e_2,x_2)=0.
\end{equation}
Suppose the $x_i$ belong to the p-cycle $C$ of \C..
If
$e_1,e_2$ respects $\o C$ then wlog the p-cycle corresponds to $C,e_2$, and
\begin{equation}
\label{DelCResEqn}
\Delta(e_1,x_1)+\Delta(e_2,x_2)=w(C_{x_1}).
\end{equation}
In the remaining case,
i.e., $e_1,e_2$ does not respect $\o C$,
\begin{equation}
\label{DelCNoResEqn}
\Delta(e_1,x_1)+\Delta(e_2,x_2)\ge 2(\omega+|w|(E-\gamma(C))).%=\omega.
\end{equation}

\yclaim 1
{\em Let $\o S$ be a cycle of $\o G$.  If $\o S$ respects $\o {\C.}$ then
$\o w(\o S)=w(S)$ for $S$ the preimage of $\o S$.  If $\o S$ does not respect
$\o {\C.}$  then $\o w(\o S)\ge 2\omega$.}

\bproof
Let $\C.\R.$ ($\C.\N.$) contain the p-cycles of \C.
that are respected (not respected) by
$\o S$, respectively.
Let $CX=\bigcup\set{C_x}{x = x_1 \text{ in } \eqref{DelCResEqn} \text{ for }
C \in \C.\R.}$.
Then
\eqref{DelVEqn}--\eqref{DelCNoResEqn}
imply
\begin{equation}
\label{CWeightEqn}
\o w(\o S) \ge w(\set{e}{e\in \o S \cup CX} ) +
\sum \set{2(\omega +|w|(E-\gamma(C)))} {C\in \C.\N.}.
\end{equation}

\noindent
Here we use the fact that the $2\omega$ terms cancel
on the 2 edges incident to a cycle of \C.\R. (this property actually depends on
our assumption that $t$ has a unique incident edge).

When $\o S$ respects $\o{\C.}$, i.e., $\C.\N.=\emptyset$,
\eqref{CWeightEqn} holds with equality, and we get the claim.
Suppose $\o S$ does not respect $\o {\C.}$. Then choosing $B$ as any
p-cycle of $\C.\N.$, \eqref{CWeightEqn} implies
$\o w(\o S) \ge w(\set{e}{e\in \o S \cup CX} ) +
2(\omega +|w|(E-\gamma(B))) \ge 2\omega$,
giving the claim.
\ecproof

Claim 1 implies  property P1.

\yclaim 2 {\em Let $\o S$ be a $vt$-path in $\o G$. If $\o S$ does not
  respect $\o {\C.}$ then $\o w(\o S)\ge \omega$.  If $\o S$ respects
  $\o {\C.}$ let $S$ be the preimage of $\o S$.  If $v\notin V(\C.)$
  then $\o w(\o S)=w(S)$.  If $v\in V(\C.)$ then $\o w(\o
  S)=w(S)-2\omega$.}

\bproof
$\o S$ satisfies a version of (\ref{CWeightEqn}) that accounts for the
term $\Delta(e_1,v)$ for edge $e_1=\delta(v,\o S)$.  We examine
several cases.

Suppose $\o S$ respects $\o{\C.}$.  If $v\notin V(\C.)$ then
(\ref{CWeightEqn}) holds with equality, giving the claim.  If $v\in
V(\C.)$
then \C. contains a p-cycle $C,e_1$ with $v\in V(C)$.
$\o w(\o S)$ contains an extra term
$\Delta(e_1,v)=-2\omega$, again giving the claim.

Suppose $\o S$  does not respect $\o{\C.}$.
If $v\notin V(\C.)$ then
 (\ref{CWeightEqn}) holds unmodified. As in Claim 1,
$\o w(\o S)\ge 2\omega$, giving the current
 claim.
So suppose
$v\in V(B)$ for $B\in \C.$. If $e_1$ does not respect $\o B$
$\o w(\o S)$ contains an extra term
$\Delta(e_1,v)=2\omega +w(B_v)\ge \omega +|w|(E-\gamma(B_v))$,
giving the claim. In the remaining case
$e_1$ respects $\o B$
and
$\o S$ does not respect some
$\o A\ne \o B$. The right-hand side of  (\ref{CWeightEqn}) contains the extra term
$\Delta(e_1,v)=-2\omega$, and the term for $A$ is at least
$3\omega + 2|w|(E-\gamma(A))$. These two contributions
sum to $\ge \omega+|w|(E-\gamma(A))$. Thus the right-hand side
of (\ref{CWeightEqn}) is $\ge \omega$, as desired.
\ecproof

\yclaim 3 {P2 holds every iteration.}

We argue by induction on the number of iterations.
Consider an iteration for the p-cycle $C,cc'$.
%, with $B_i$ as defined in P3.
Let \gm.,\wm. (\gp.,\wp.) be the graph and weight function
 immediately before (after) $C$ is contracted, respectively.
For greater precision, if $H$ is
\gm. or \gp. and $z$ is a vertex of $H$,
let $P(z,H)$ denote the shortest $zt$-path in $H$.
Take any $x\in V(G)$. Let $P= P(\o x, \gp.)$.
Note that $P_x$ continues to denote the shortest $xt$-path in $G$, and
for P2 we want to establish the relationship between $P$ and $P_x$.
\C. denotes the family of contracted vertices in \gp., i.e., it includes $C$.

First assume either $x\notin V(\C.)$ or $x=b$ for some p-cycle $B,bb'$ of
$\C.$ ($x=c$ is a possibility).
Let $\delta$ be 0 ($2\omega$)
if $x\notin V(\C.)$ ($x=b$) respectively.
Let $Q=P(\o x, \gm.)$.
Lemma \ref{spRespectLemma} shows $Q$ respects $C$.
Thus  $Q$ has an image $Q^+$ in \gp.
that respects $\o C$.
The inductive assumption of P2 in \gm. shows
$P_x$ is the preimage of $Q$. (For $x=c$,
$\o x$ in \gm. may be a vertex or a contracted cycle, and we use
the appropriate assertion of P2.)
Thus
the optimality of $P_x$ implies
it is the preimage of $Q^+$. Thus Claim 2 shows
\[\o w^-(Q)=\o w^+(Q^+)=w(P_x)-\delta.\]

Since $\omega> w(P_x)$, Claim 2 shows $P$ respects $\o {\C.}$ and
\[\wp.(P)=w(P^-)-\delta\] for  $P^-$ the preimage of $P$.
Since $P^-$ is an $xt$-path,
\[w(P^-)\ge w(P_x).\]
Combining the inequalities gives $\wp.(Q^+)\le \wp.(P)$. Thus
$Q^+=P$. So as asserted by the first part of P2, $P_x$
is the preimage of $P_{\o x}$.

Also, as in the second assertion of P2, every
p-cycle $B,bb'$ of $\C.$
has
$P_b$ and $P({\o B},\gp.)= P({\o b},\gp.)$
both
 starting with edge $bb'$.
This follows since
$P({\o b},\gm.)$ starts with $bb'$ (by definition if $b$
is not in a contracted vertex of \gm., else by  P2 in \gm.)
and $P_b$ is the preimage of
both $P({\o b},\gm.)$ and $P({\o b},\gp.)$.

%Lemma \ref{sp2.2} , and

Finally  the last assertion of P2 follows since
any $y\in V(B)$ has $\o y=\o b$.
\ecproof

\yclaim 4 {P3 holds in every iteration.}

\bproof
By definition \[\o\zeta(uv)=
\o w(P_{\o u})+ \o w( P_{\o v})\oplus \o w(uv)=
(\o w(P_{\o u})\oplus\Delta(uv,u))+
(\o w( P_{\o v})
\oplus\Delta(uv,v))
\oplus w(uv)\]
for some $\oplus\in \{+,-\}$.
Since $uv$ is an edge of $\o G$, P2 shows
$uv\in P_u$ iff $uv\in P_{\o u}$. Hence the version of this formula
for $\zeta(uv)$ uses the same sign $\oplus$ as $\o \zeta(uv)$.
%The rest of the argument uses the same logic in all cases:
We evaluate  $\o\zeta(uv)$ using the formula, with
Claim 2 %of Lemma \ref{spContractLemma}
providing $\o w(P_{\o u})$
 and the definition of $\Delta(uv,u)$
giving its value, as follows.

Suppose $u\notin V(\C.)$.  $P_u$ is the preimage of $P_{\o u}$ by
P2. % and the definition of preimage.
 So
\[\o w(P_{\o u})\oplus\Delta(uv,u)=w(P_u)\]
since $\o w(P_{\o u})=w(P_u)$, $\Delta(uv,u)=0$.

Suppose $u\in V(\C.)$, say $u\in V(C)$ for the p-cycle $C,cc'$.
$P_c$ is the preimage of $P_{\o u}$ by
P2. % and the definition of preimage.
Claim 2 shows $\o w(P_{\o u})=w(P_c)-2\omega$.
If $uv \notin P_u$ then
\[\o w(P_{\o u})+ \Delta(uv,u)=w(P_u)\]
since $\Delta(uv,u)=2\omega+w(C_u)$, and $P_u=C_u\cup P_c$ by
P2 and the optimality of $P_u$.
If $uv \in P_u$ then
\begin{eqnarray*}
\o w(P_{\o u})- \Delta(uv,u)&=&w(P_u),\\
\o w(P_{\o u})+ \Delta(uv,u)&=&w(P_u)-4\omega
\end{eqnarray*}
since P2 implies $u=c$ and $\Delta(uv,u)=-2\omega$.

%$\o w(P_{\o u})+\Delta(uv,u)=(w(P_u)-2\omega)+(-2\omega)=w(P_u)-4\omega$.

The alternatives of P3 all follow, by
combining the equations with $-$ signs for $uv\in P_u\cap P_v$
and $+$ signs in all other cases.
\xecproof
\end{proof}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%END
\iffalse
The remaining case is for the root node \V. of \T., with \V.
 a tree node. Let $\o G$ be the final acyclic graph.
Let $\o x$ be the image of $x$ in $\o G$,
%If $\o x$ is the vertex $x$ ($x\notin V(\C.)$) P2 shows
%$P_x$ is the preimage of $P_{\o x}$, as desired.
with $\o x$ the contracted cycle $C,cc'$.
P2 shows $P_c$ is the
preimage of $P_{\o C}$. Thus \T. specifies the desired path $p(c,\V.)$.
The first assertion of P2 shows this extends to any vertex $x\in V(C)$.
\ecproof
\end{proof}

\fi


\iffalse
\bproof
We wish to show that
$xx$ is chosen as the minimum weight p-cycle of some iteration.
The following argument takes place in the contracted graph
$\o G$ of the iteration, but for notational convenience we omit
bars, e.g., we write $w$ rather than $\o w$.

For the purpose of contradiction, suppose that
$x$ gets contracted in a p-cycle $C,cc'$
where, in the notation of \eqref{WeightSEqn},
\[w(S)=\zeta^*<\zeta(xx).\]
(The inequality follows since $xx\notin P_x\oplus P_x=\emptyset$
so $xx$ is always considered
in the definition of $E^*$ and $\zeta^*$.)
First assume $x\ne c$.
Let $x$ be on edge $xy$ of $C$.
Using the notation of \eqref{BxEqn},
$S$ is the disjoint union of $B_x$ and $B'_x$.
Using  symmetry, $w(P_x)\le w(B_x)<w(B'_x)$.
This implies $w(xx)+w(P_x)<w(B'_x)$.
(Proof: In the definition of the perturbed weight function
we can assume
$\epsilon^i>\sum_{j>i}\epsilon^j$. Thus the perturbed weight function
breaks ties lexically.  The loop $xx$
is ordered after any edge of $G$, so it cannot reverse
the ordering  $w(P_x)<w(B'_x)$.)
Hence
\[\zeta^*(xx)=w(xx)+2w(P_x)<w(B_x)+w(B'_x)=
w(S),\] contradiction.
The case $x=c$ is similar:
Since $G$ is conservative
$w(xx)<w(C)$, so
$w(cc)+2w(P_c)<w(C)+2w(P_c)=w(S)$.
\ecproof
\fi


\iffalse
The perturbed weight function implies  $C$ contains every edge of $E^*$.
So it remains only to show \i for edge $cc'$.
Since $c\in C$, \ii  shows that
$P_c$ is the $ct$-path in $S$.
If $cc'\in P_c -P_{c'}$ then
$P_{c'}$ is a subpath of $P_c$ (Lemma \ref
{SimpleLemma}). Thus $\zeta(cc')=2w(P_c)$.
So $\zeta^*=w(S)= 2w(P_c)+w(C)$ with $w(C)>0$
gives \xii.
\fi

\iffalse %++++++++++++++++++++++++++++++++++++++++++++++++++++++
\yclaim 2 {\it There are no paths of type (c).}

\bproof
Assume the contrary, i.e., the above set $X$ is nonempty.
%Let $C$ be the circuit $T\cup uv$.
$|X|$ is even, i.e., the vertices of $X$ divide the edges of
$C$ into an even number of segments $C_i$.
Partition the edges of $C$  into 2 sets $\C._1, \C._2$,
each consisting of alternate segments  $C_i$.
Partition the edges of the type (c) paths into 2 sets $\P._1,\P._2$,
each consisting of 1 copy of each type (c) path $P_j$.
Now the edges of type (a) and (c) are partitioned into
the two sets
 $\P._s\cup \C._s$, $s=1,2$.
\iffalse
Each such $C_i$ is a path.
In proof, suppose $C_i$ contains
a cycle $A$, with cutpoint $a$ of $C$ (by Claim 2).
$A$ is not entirely contained in one
path $P_u, P_v$, so some $a'\in A-a$ is on edge of
$A\cap P_u$ and an edge of $A\cap P_v$.
$a'$ has degree 2 in $C$ (Claim 2).
Thus $a'\in X$, contradiction.
\fi


{\def\Q.{\P.\C.}
Let $\Q.$ be one of the subgraphs
$\P._s\cup \C._s$.
Observe that each vertex $x$ has $d(x,\Q.)$ even:
If $x$ is interior to a $P_j$ then $d(x,\Q.)=2$.
If $x$  is the end of a $P_j$ then it
is the end of a corresponding $C_i$,
so again $d(x,\Q.)=2$.
%, or 4 if it occurs again in  $C_i$.
(It is worthwhile to  describe the case $x=u$:
We cannot have $uv\in P_u\cap P_v$, since such vertices $u$ have
$d(u,S)=2$ and so $u\notin X$.
So $uv\notin P_u\cup P_v$. Furthermore
the first edge of $P_u$, say $f$, belongs to $P_v$,
and  $\Q.\cap \delta(u)$ consists of  $f$ plus
either the other edge of $P_v\cap \delta(u) $ or $uv$.)
Any other $x$ has 1 or 2 occurrences in \Q., both  interior to  $C_i$'s.
(2 occurrences may correspond to $x$ occurring twice in some $C_i$,
 or once in two different $C_i$'s.)
Thus $d(x,\Q.)\in \{2,4\}$.

We conclude that each connected component of
$\Q.$ is a circuit (the construction ensures
the circuit is edge-simple, since
any edge of $G$ occurs at most once in
$\Q.$). As such \Q.
can be partitioned into cycles, and so  has
nonnegative weight.
In fact the perturbation implies the weight is positive.
}

\iffalse
Its edges  form a subgraph of even degree  vertices
(each vertex is interior to exactly one
$P_i$, one or two some $C_j$'s, or it is the end of
exactly 1 $P_i$ and 1 $C_j$).
Thus
$\P._1\cup \C._1$ can be partitioned into cycles of $G$, so it has
nonnegative weight.
In fact the perturbation implies the weight is positive.
The same holds for $\P._2\cup \C._2$.
\fi

One of these circuits, call it $B$,  contains vertex $b$.
Form a subgraph $S'$ by using
the circuit $B$
and the type (b) path of $S$ from $t$ to $b$.
$X\ne \emptyset$ implies $w(S')<w(S)$.

Let
$B$ contain an edge $xy \notin P_x\oplus P_y$ (Corollary \ref{ForestCor}).
\iffalse
Suppose $xy\notin P_x\cup P_y$. Thus
$\zeta(xy)=w(P_x)+ w( P_y)+ w(xy)$.
\fi
Let $B_x$ ($B'_x$) be the $xt$-trail contained in $S'$ that avoids (contains)
$xy$, respectively.
%$B_x$ contains an $xt$-path $B'_x$, and
%$w(B'_x)\le w(B_x)$ (as $w$ is conservative).
Define $B_y$ and $B'_y$
similarly.
Then
\begin{equation}
\label{BxEqn}
w(B_x) +w(B_y)+w(xy)=
w(B'_x) +w(B'_y)-w(xy)=
w(S')<w(S)=\zeta^*.
\end{equation}
The definition of $\zeta(xy)$ shows it is at most
the first expression of \eqref{BxEqn}
if $xy\notin P_x\cup P_y$,
or the second expression  if $xy\in P_x\cap P_y$.
Thus $\zeta(xy)<\zeta^*$, contradiction.
\ecproof

\yclaim 3 {\it A vertex on 4 edges of $C$ is a cutpoint of $C$.}

\bproof
Suppose vertex $a$ is on 4 edges of $C$.
So it is on 4 nonloop edges of $T$.
In the definition of $T$ (Claim 1)
we can choose $T$ to have smallest possible length.
Let the 4 edges of $\delta(a)$ occur in the order $e_1,e_2$, \ldots, $e_3,e_4$
along $T$, and let $A$ denote the subtrail
$e_2,\ldots, e_3$. Wlog let $e_1\in P_u$.
This implies $e_4\in P_u$, else we could delete $e_2,\ldots, e_3$ from $T$.
Thus $e_2,e_3\in P_v$.
Suppose that after $e_4$  $T$ returns to a vertex (degree 4) vertex $a'$ of $A$,
and leaves $a'$ on  edge $f$. $A$  is the union of 2
$aa'$-trails. Let $A'$ be the $aa'$-trail
such that $e_1$, $A'$, $f$ has alternations
at $a$ and $a'$.
$A'$ exists, since the two edges of $A\cap \delta(a')$
alternate.
$A'$ gives a shortcut of $T$.
\ecproof


\iffalse
\yclaim 3 {\it There are no paths of type (c).}

\bproof
Assume the contrary, i.e., the above set $X$ is nonempty.
%Let $C$ be the circuit $T\cup uv$.
The vertices of $X$ divide the edges of
$C$ into an even number of segments $C_i$.


Each such $C_i$ is a path.
In proof, suppose $C_i$ contains
a cycle $A$, with cutpoint $a$ of $C$ (by Claim 2).
$A$ is not entirely contained in one
path $P_u, P_v$, so some $a'\in A-a$ is on edge of
$A\cap P_u$ and an edge of $A\cap P_v$.
$a'$ has degree 2 in $C$ (Claim 2).
Thus $a'\in X$, contradiction.

Partition the edges of $C$  into 2 sets $\C._1, \C._2$,
each consisting of alternate segments  $C_i$.
Partition the edges of the type (c) paths into 2 sets $\P._1,\P._2$,
each consisting of 1 copy of each type (c) path.

By symmetry,
consider  $\P._1\cup \C._1$.
Each vertex has even degree in this subgraph
(each occurrence of a vertex is interior to a $C_i$,
interior to a $P_j$, or the end of a  $C_i$ and a $P_j$).
Thus each connected component of
$\P._1\cup \C._1$ is a circuit. As such it
can be partitioned into cycles, and so  has
nonnegative weight.
In fact the perturbation implies the weight is positive.
The same holds for $\P._2\cup \C._2$.


\iffalse
Its edges  form a subgraph of even degree  vertices
(each vertex is interior to exactly one
$P_i$, one or two some $C_j$'s, or it is the end of
exactly 1 $P_i$ and 1 $C_j$).
Thus
$\P._1\cup \C._1$ can be partitioned into cycles, so it has
nonnegative weight.
In fact the perturbation implies the weight is positive.
The same holds for $\P._2\cup \C._2$.
\fi

One of the these circuits, call it $B$,  contains vertex $b$.
Let $P$ be the type (b) path of $S$ from $t$ to $b$.
Form a subgraph $S'$ by using $P$
and the circuit $B$.
Obviously $w(S')<w(S)$.

Let
$B$ contain an edge $xy \notin P_x\oplus P_y$ (Corollary \ref{ForestCor}).
Suppose $xy\notin P_x\cup P_y$. Thus
$\zeta(xy)=w(P_x)+ w( P_y)+ w(xy)$.
Let $B_x$ be the $xt$-trail contained in $S'$ that avoids $xy$.
%$B_x$ contains an $xt$-path $B'_x$, and
%$w(B'_x)\le w(B_x)$ (as $w$ is conservative).
Define $B_y$ %and $B'_y$
similarly.
Then
\[\zeta(xy)\le %w(B'_x) +w(B'_y)+w(xy)\le
w(B_x) +w(B_y)+w(xy)=w(S')<w(S)=\zeta^*,
\]
contradiction. A similar contradiction holds when
 $xy\in P_x\cap P_y$ (the term $+w(xy)$ becomes $-w(xy)$ in the above
inequalities).
\ecproof
\fi


\iffalse
\bproof
Assume the contrary, i.e., the above set $X$ is nonempty.
%Let $C$ be the circuit $T\cup uv$.
The vertices of $X$ divide the edges of
$C$ into an even number of segments $C_i$.
Each such $C_i$ is a path.
In proof, suppose $C_i$ contains
a cycle $A$, with cutpoint $a$ of $C$ (by Claim 2).
$A$ is not entirely contained in one of the
paths $P_u, P_v$, so some $a'\in A-a$ is on edge of
$A\cap P_u$ and an edge of $A\cap P_v$.
$a'$ has degree 2 in $C$ (Claim 2).
Thus $a'\in X$, contradiction.

Partition the edges of $C$  into 2 sets $\C._1, \C._2$,
each consisting of alternate segments  $C_i$.
Partition the edges of the type (c) paths into 2 sets $\P._1,\P._2$,
each consisting of 1 copy of each type (c) path.

By symmetry,
consider  $\P._1\cup \C._1$.
Its edges  form a subgraph of degree 2 vertices
(each vertex is interior to some $C_i$ or some $P_j$, or it is the end of
exactly 1 $C_i$ and 1 $P_j$).
Thus each connected component of
$\P._1\cup \C._1$ is cycle, so it has
nonnegative weight.
In fact the perturbation implies the weight is positive.
The same holds for $\P._2\cup \C._2$.

One of the these cycles, call it $B$,  contains vertex $b$.
Let $P$ be the type (b) path of $S$ from $t$ to $b$.
Form a subgraph $S'$ by using $P$
and the cycle $B$.
Obviously $w(S')<w(S)$.

We obtain the desired contradiction by showing
$B$ contains an edge $xy \notin P_x\oplus P_y$.
In fact we show the edges $xy \notin P_x\oplus P_y$ are acyclic.

\ecproof
\fi

\yclaim 4 {\it $C$ is a cycle.}

\bproof  Suppose $C$ contains a
degree 4 vertex $a$. By Claim 3 we can assume
$C$ contains a cycle $A$ at $a$.
$A$ is not contained in one path $P_u$, $P_v$.
So $A$ has a vertex $z$ of degree 2 in $C$ where the 2 edges at $z$ alternate.
In fact $A$ has at least 2 such vertices. (If there is just one alternation,
as in Claim 3 $T$ can be shortcut.) At least one of these vertices is on
a type (c) path (the other can be on the type (b) path).
This contradicts Claim 2.
\ecproof

\fi %++++++++++++++++++++++++++++++++++++++++++++++++++++++

\iffalse
Furthermore for a p-cycle $B_i,b_i b'_i$, P2 shows $\o E(P_{\o B_i})$
starts with $b_ib'_i$.
 P2 shows any $x\in V(B_i)$ has $P_{\o B_1}$ is the image of $P_c$ and
 again . In particular $P_c$ starts with $cc'$, i.e., the second
 assertion of P2 hol

%It remains to show the first two assertions of P2 hold after
%$C$ is contracted.


$P_u$ is the preimage of $P_{\o u}$, by
P2 and the definition of preimage.

$P_c$ is the preimage of $P_{\o u}$, by
P2 and the definition of preimage.

 $P_u=C_u\cup P_c$ by
P2 and the definition of $C_u$.
\fi

\iffalse
P4 for $uv \notin P_u\cup P_v$ follows.
\case{$uv \in P_u\cap P_v$}
P4 for $uv \in P_u\cap P_v$ follows.

\case{$uv \in P_u- P_v$}
First observe
$\o w(P_{\o v})+ \Delta(uv,v)=w(P_v)$.
For
$v\in V(\C.)$ it follows as in the first case.
\fi

\iffalse
The inductive assumption of P2 in \gm. shows
the first two assertions of P2 in \gp..

Claim 2 shows that $P$ respects $\o {\C.}$.
Thus $P$ corresponds to an $\o x t$-path $P^-$ in \gm..
The definition of $\o w$ shows these 2 paths have the same weight,
i.e., $\o w^-(P^-)=\o w^+(P)$.

By definition $\o w^-(Q)\le =\o w^-(P^-)$.
Thus $\o w^+(Q+)\le \o w^+(P)$.
Since $Q^+$ is an $\o x t$-path in \gp., we get
$Q^+=P$.
The inductive assumption of P2 in \gm. shows
the first two assertions of P2 in \gp..
P3 shows

To show the last assertion of P2,
apply P3 to $C,cc'$.
If $c\notin V(\C.)$ P3 shows
$P_c$ is the preimage of $P(\o C,\gm.)$.
Similarly if $c\in V({\C.})$,
say $c\in V(B_1)$,
 P2 shows
$P_c$ is the preimage of
 $P({\o B_1},\gm.) $.
, is the image of $P_c$ and $c'\notin V(C)$
gives the last assertion of P2.
---------------------------------

Claim 2 shows that in general,
we minimize $\o w (\o P)$ by minimizing $w(P)$ for $P$ the preimage of $\o P$.

This implies $P_c$ is the preimage of $P(\o C, \gp.)$.
This gives Claim 2 for $x\in V(C)$.


For $\o x \ne \o C$,
P2 shows before contraction $P(\o x, \gm.)$ is the image of $P_x$.
Lemma \ref{spRespectLemma} shows immediately
after contraction $P(\o x,\gp.)$ is the image of $P_x$.
So Claim 2 shows this is preserved when we switch to $\o w$.
This
gives the first assertion of P2 after contraction.
---------------------------

To show P2 take any $x\in V(G)$. First suppose
 $\o x \ne \o C$. P2
shows $P(\o x, \gm.)$ is the image of $P_x$.
Lemma \ref{spRespectLemma} shows
$P(\o x, \gm.)$ respects $C$.
is the image of $P_x$.

in \gp. with weights $\o w$,
the minimum weight $\o x t$-path
respects $C$, and the $\o x t$-paths of \gm.


immediately
after contraction $P(\o x,\gp.)$ is the image of
 $P(\o x, \gm.)$, so it is the image of $P_x$.
Claim 2 shows $P_{\o x}$ does not change when we switch
to weight funcsion $\o w$.


Further suppose $x\notin V(\C.)$.
\fi

\iffalse
{The rest of the derivation mimics f-factors, and
isn't given.}
This includes a simple analog  of Lemma \ref{sp2.2}
that applies to every iteration of the shrinking procedure,
not just the first.

The definition of $z$ from $\zeta$ is the same as $f$-factors:

Let $p$ be the parent function in \T..
\begin{equation}
\label{DualDefnEqn}
\begin{array}{lcll}
%y(v)&=&-w(F_ v)\hspace{102pt}v \in V,\\
%\end{array}\\
%\]
%\[
%z(G)&=&\zeta(G)\\
%z(B) &= &\zeta(B)-\zeta(p(B))&B \mbox{ a blossom }\ne G.
%\begin{array}{lcll}
z(C) &= &
\left\{
\begin{array}{ll}
\zeta(C) &\text{$C$ is a maximal cycle node in  \T.},\\
\zeta(C)-\zeta(p(C)))&C \mbox{ a nonmaximal cycle node.
%\\
%0&\mbox{otherwise.}
}
\end{array}
\right.
\end{array}
%\]
\end{equation}
\fi


\iffalse
Continue with the $uv$-subgraph of Lemma \ref{sp2.2}.
Take
 any vertex $a\notin C$ whose path
$P_a$ contains a vertex of $C$.
Let $xy$ be the first edge of $P_a \cap \delta(C)$,
say $x\in C \not\ni y$. Then $P_x\con P_a$. This follows from
the argument at the start of Claim 1.

For uniformity, in the given graph add a loop $xx$
of weight 0 at each vertex $x\ne t$.
Now every iteration of the shrinking procedure
shrinks a cycle $C$ (perhaps $C$ is a loop).
The first iteration of the shrinking procedure
shrinks the cycle $C$. $C$, with children $V(C)$, becomes a node of
the shortest path structure.
Let $\overline G$ denote the new graph, with
$\overline C$ the image of $C$.

We define a shortest path problem on $\overline G$ as follows.
The new sink is $t$, or  $\overline C$ if
$t\in C$. If $t\notin C$
add a loop at $\overline C$ to $\overline G$.
Modify the weights of edges incident to $C$
to reflect this fact, and subpaths within $C$, as follows:
Let $M= 4\sum {w(e)}{e\in E(G)}$.
$\overline C \overline C$ gets weight $M$.
For $x\in C$ let $P_{x,b}$ be the $xb$-subpath of $P_x$.
An edge  $xy\in \delta(C)-bb'$, say  $x\in C \not\ni y$,
 gets new weight
$w(e) +w(P_{x,b}) +M$.

In the new graph, for any vertex $x\notin C$
the shortest $xt$-path has weight increased by $M$.
(The definition of $M$ ensures the path contains just one edge
of   $\overline C-bb'$.  The shortest $\overline C t$-path has the weight
of the shortest $bt$-path (in $G$) increased by $M$.

Lemma \ref{sp2.2}
holds in $\overline G$. The proof is the same.

Finally we define the $z$ function for the shortest path structure.
Each cycle $C$ that gets contracted is a node of the generalized tree
\T..
Let $\zeta(C)$ denote the value $\zeta^*$ when $C$ is contracted.
(Ignore the terms involving $M$.)
If $C$ is


Let $p$ be the parent function in \T..
\begin{equation}
\label{DualDefnEqn}
\begin{array}{lcll}
%y(v)&=&-w(F_ v)\hspace{102pt}v \in V,\\
%\end{array}\\
%\]
%\[
%z(G)&=&\zeta(G)\\
%z(B) &= &\zeta(B)-\zeta(p(B))&B \mbox{ a blossom }\ne G.
%\begin{array}{lcll}
z(C) &= &
\left\{
\begin{array}{ll}
\zeta(C) &\text{$C$ is a maximal cycle node in  \T.},\\
\zeta(C)-\zeta(p(C)))&C \mbox{ a nonmaximal cycle node.
%\\
%0&\mbox{otherwise.}
}
\end{array}
\right.
\end{array}
%\]
\end{equation}

As desired
$z$ is nonpositive except for maximal nodes.
An edge $xy$ that gets shrunk
when $C$ is contracted has  $\zeta(xy)\ge \zeta(C)$, with
equality for edges of $C$.


%\ge \sum {C covers xy}$, with equality if
%$xy $ belongs to the shrunk cycle.
So \eqref{DomEqn} holds.
\fi


\iffalse
%%%%%%%%%%%% !!!! %%%%%%%%%%%%%%%%
If $bb'\in P_b \cap P_b'$ then
$P_b'$ is not a subpath of $P_b$, so $w(P_b')< w(P_b-bb')$.
Thus $\zeta(bb')< 2w(P_b) -2w(bb')$.
\fi
\iffalse
We view the shortest path problem as an f-factor problem as follows.
An {\em sp-graph} $(G,t,w,f)$ consists of a graph $(G,t,w)$
where there is
a self-loop of weight 0 at every vertex $v\ne t$,
and $f$ gives
degree-constraints with
$f(v)=2$ for $v\ne t$ and $f(t)=1$.

An sp-graph is clearly $f$-critical.
Specifically for any $v\in V$, an $f_v$-factor $P$
consists of a $vt$-path $P^-$ and a collection of vertex disjoint
cycles over the vertices not in $P^-$. We shall use the $P,P^-$ notation
(for any $f_v$-factor $P$) in the ensuing discussion.
A  shortest $vt$-path corresponds
to a  minimum $f_v$-factor. Here we use the fact that
weights are conservative. Thus a minimum $f_v$-factor $P$
consists of a shortest $vt$-path $P^-$ and a collection of
weight 0 cycles, which wlog are all loops.



The proof for the general case modifies the above version of Bellman's inequality using a laminar family. Consider a laminar family \B. of subsets of
$V$, with  $V\in \B.$. In addition each
$B\in \B.$ with $t\notin B$ has an associated edge $I(B)
\in \delta(B)$.  Say $B$ {\em covers} every edge in $\gamma(B)\cup I(B)$.
Observe that $B$ covers at most $|B|$ edges of any $f_v$-factor $P$.
(If $P^-$ be the $vt$-path of $P$,





We will show that executing the shrinking procedure of \cite{G}
on this graph constructs the desired shortest path structure.
Let $SG$ be an sp-graph some of whose loops
can be blossom loops (formed by the shrinking procedure).

CHOICE OF UNIFACTOR?

\begin{lemma}
\label{StrucLemma}
\end{lemma}

\begin{lemma}
$SG$
has a minimum irredundant $2f$-unifactor
whose
blossom $B$ has
one of the following two forms, with $CH(B)=\emptyset$:

\i $C(B)=\{bb\}$  and
\[|I(B)|=
\begin{cases}
0&b=t\\
1&b\ne t.
\end{cases}
\]

\ii For some cycle $C$ of $\ge 3$ vertices, each of which is a blossom vertex, and some
vertex $b\in C$, $C(B)=C\cup \set{vv}{v\in C-b}$, with
$I(v) \con C$ for each
$v\in C-b$
and
$I(B)=I(b)$.
\end{lemma}

\begin{proof}
In
a $2f$-unifactor of an sp-graph, $t$ has degree 2 and all other vertices
have
degree 4.


Note that \i and \ii both describe a blossom:
For \xi, a loop $bb$ is the odd circuit of a $2f$-unifactor
whose multiplicity 2 edges
form a path from $t$ to $b$ plus a loop at every nonpath vertex.
$I(B)$ is the edge of the path incident to $b$.
(If $b=t$ the path has length 0 and $I(B)=\emptyset$.)
For \xii, note that $C(B)$ is an odd circuit.
The unifactor's multiplicity 2 edges are similar to \xi.
 Definition \ref{BTreeDfn} shows  we have $I(B)=I(b)$.

Now let $U$ be a minimum irredundant $2f$-unifactor, with
$C$ its cycle of multiplicity 1 edges.
Choose $U$ so that $C$ has the smallest length possible.
Recalling that a vertex has degree 4 (or 2 for $t$) in $U$,
we see that $U$  has
three types of edges of  multiplicity 2:
(a) a multiplicity 2 path $P$ from $t$ to some $b\in C$ (possibly $t=b$);
(b) a multiplicity 2 path joining two distinct vertices $v,v'\in C-b$;
(c) a multiplicity 2 loop $vv$ for
every vertex
$v$ not in $P\cup C$ or a type (b) path
(this is  wlog, since weights are conservative).

If $C$ is a loop we have shown $B$ has the form of \xi.
So suppose $C$ is not a loop.

\xclaim {$U$ has no  type (b) path.}

\bproof
Assume $U$ has type (b) paths.
The ends of these  paths divide the edges of
$C$ into an even number of segments $C_i$.
Partition the edges of $C$  into 2 sets $\C._1, \C._2$,
each consisting of alternate segments  $C_i$.
Partition the edges of the type (b) paths into 2 sets $\P._1,\P._2$,
each consisting of 1 copy of each type (b) path.

By symmetry,
consider  $\P._1\cup \C._1$.
Its edges of form a regular subgraph of degree 2
(each vertex is interior to some $C_i$ or $P_j$, or it is the end of
exactly 1 $C_i$ and 1 $P_j$).
Thus $\P._1\cup \C._1$ is a  union of disjoint
cycles, each with nonnegative weight.
The same holds for $\P._2\cup \C._2$.

One of the these cycles, call it $B$,  contains vertex $b$.
Let $P$ be the type (a) path of $U$ from $t$ to $b$.
Form a unifactor $U'$ by using $P$,
the cycle $B$, and a loop $vv$  at every vertex $v\notin
P\cup B$.
$U'$ has no greater weight than  $U$ and fewer edges, contradicting the choice
of
$U$.
\ecproof

Now we show the blossom $B$ of $U$ satisfies \xii.


Suppose some vertex $v\in C$ is not a blossom vertex.
The edges of $C$ can be partitioned into two $vt$-paths
$C_1,C_2$, with $w(C_1)\le w(C_2)$.
(If $v=b$ take $C_1=\emptyset$, $C_2=C$, and use $0\le w(C)$.)
 This implies
$2w(C_1)\le w(C)$. Let $U'$ be the unifactor
consisting of the  circuit  $vv$, the multiplicity 2 $vt$-path
formed from
$P$ and $C_1$, and loops at all other vertices.  Since $w(U')\le w(U)$,
$U'$ can be chosen as the unifactor of the lemma, and it has form \xi.

Now we can assume every $v\in C$ is a blossom vertex.
Every $v\in C-b$
is on a loop
$vv\in C$ (by the claim,  with $f(v)=2$,
and Corollary
\ref{AMaxUnifactorCorollary}).
Thus $C$ contains the blossom loop $vv$.


 Definition \ref{BTreeDfn} shows that any $v\in C$ has
$I(v)\con C\cup CH(B)\cup I(B)$.  Our description of $U$ shows
$CH(B)=\emptyset$ and $I(B)$ consists of at most one edge,
the edge of $P$ incident to $C$ (if it exists).
So any
$v\in C-b$
has $I(v) \con C$. Consider vertex $b$.
Recall $f(b)=|I(b)|+1$. So
if $b=t$ then $I(b)=\emptyset=I(B)$.
If $b\ne t$ then $|I(b)|=1$, and since
$bb$ is not an edge of $C$,
 Definition \ref{BTreeDfn} implies $I(b)\cap C=\emptyset$.
Thus $I(B)=I(b)$.
We conclude $B$ has form \xii.
\end{proof}

Consider a step of the blossom-shrinking procedure that starts
with an sp-graph $G$ and contracts a blossom $B$ to form graph
$\o G$. We claim $\o G$ is
an sp-graph.

We conclude that every blossom is of form \i or \xii.

It is easy to see the blossom tree gives the shortest path structure.

\iffalse
\begin{lemma}
\label{BTreeLemma}
Consider any blossom $B$ in

\i $(V(B), I(B))$ is an $f$-odd pair.

\ii An edge of $CH(B)$ that has
$B_i$ as an end belongs to
$I(B_i)\cup I(\o B_i \o B_i)$.
\end{lemma}



\begin{proof}
\end{proof}

Now we check that
the blossoms of our construction
give a forest satisfying Definition \ref{BTreeDfn}.
For a vertex $v$, the minimal blossom
$B$ containing $v$ has $f(v)+1$ edges
incident to $v$ in $C(B)\cup CH(B)\cup I(B)$
(Lemma \ref{UnifactorLemma}
and Corollary \ref{MaxUnifactorCorollary}).
So deleting the circuit edges gives
the set $I(v)$ of the definition, and also
property \ii is satisfied.


%two required properties in blossom $B$
%(i.e., property \i and the consistency property).

To check an interior node $B$ we
introduce notation that will be handy later on.
Recall $B$ is created as the elementary blossom
of a maximum irredundant unifactor. Let
\[
\b G.(B), \o U(B), \text{ and } \o V(B)
\]
denote the contraction of $G$ wherein $B$ is created,
the unifactor, and
the set of vertices of $\b G.(B)$ in $B$, respectively.
So $C(B)$ is the circuit of $\o U(B)$ on $\o V(B)$,
and $CH(B)$
($I(B)$)
is the set of chords
 (incident edges) of $\o U(B)$
on this circuit, all at half multiplicity.
These sets are defined in the construction of
the elementary blossom of $\o U(B)$
(Lemma \ref{MaxUnifactorLemma}), and they are the
same-named sets in
Definition \ref{BTreeDfn}. In that definition $\o V(B)$
is denoted $\{B_i\}$ and $\o V(B)$ is the image
of
$V(B)$ in $\b G.(B)$.
As an example in Fig.\ref{NonLamFig}(b),
$\o V(B_1)$  has $B_2$ contracted to $\o B_2$, and
$C(B_1)$ is the triangle $\o B_2,d,e$.

Properties \xi--\iii of the definition
correspond to \xi--\iii of
the claim in the proof of
Lemma \ref{BlossomUnifactorLemma}.
So \xi--\iii hold
for any child $B_i$ as long as
\[I(B_i)=F_{B_i}\cap \delta(B_i).\]
This in turn holds by
Lemma \ref{WeightLemma}\ii and
Corollary \ref{RespectCor}
(specifically the lemma shows
that for any $v\in C(B_i)$,
$F_{B_i}\cap \delta(B_i)=
F_v\cap \delta(B_i)$, and the corollary
shows
$F_{v}\cap \delta(B_i)=I(B_i)$).


Lastly we  check
the equations for
$I(B)$ and $CH(B)$.
Recall the elementary blossom $B$ of a unifactor $U$
with circuit $C$
has $I(B)=(U\cap \delta(C))/2$,
$CH(B)=(U\cap \gamma(C)-E(C))/2$.
Consider a child $B_i$ of $B$ that is a blossom.
Apply Lemma \ref{BlossomUnifactorLemma} to $B_i$,
and use the above equation for
$I(B_i)$.
We get that
the
edges of $I(B)$ and $CH(B)$ with an end in $B_i$
are $I(B_i)\cap \delta(C)$
and $I(B_i) \cap \gamma(C)-E(C)$, respectively, with one possible exception:
$U-E(C)$ may contain the loop $B_i B_i$, but this loop is not in
$I(B_i)$. This occurs in alternative \i
(see the proof of the Claim of Lemma \ref{BlossomUnifactorLemma}).
It corresponds to the term
$I(\o B_i \o B_i)$ in the definition of $CH(B)$.
Finally note that
 if $B_i$ is a vertex a simpler version of this argument applies.

Next we examine the odd pair
$(V(B), I(B))$ of Lemma \ref{BTreeLemma}\i applied to our construction.
(This pair will be used to define the $z$ duals.)

\begin{lemma}
\label{I(B)Lemma}
The odd pair $(V(B), I(B))$  for a blossom $B$ covers edge $uv$ of $G$ iff
%$u,v\in V(B)$ or $uv \in I(B)$. The former holds iff
$B$ is an ancestor of both $u$ and $v$, or
%The latter holds iff
$B$ is an ancestor of exactly one of $u$, $v$
say $v$, and
$uv\in F_v$.
\end{lemma}

\begin{proof}
Clearly $u,v\in V(B)$ iff $B$ is a common ancestor of $u$ and $v$.
Consider an edge $uv$ of $G$ whose image $\bar u \bar v$ in $\b G.(B)$
belongs to
$I(B)$.
This holds iff $\bar u \bar v$ is incident to $\bar V(B)$, say
$\bar v \in \bar V(B) \not\ni \bar u$,
and $\bar u \bar v\in \o U(B)$.
The former holds iff $v\in V(B)\not\ni u$.
The latter holds iff $\bar u \bar v\in F_{\bar v}$.
Lemma \ref{WeightLemma}\ii shows this last condition is equivalent
to $u v\in F_{v}$.
\end{proof}


\iffalse
The edges of $I(B)$ have exactly one end in $V(B)$ and belong to $U(B)$.
If $v$ is the end in $V(B)$, $uv $ belongs to $U(B)$ iff it belongs
to $F_v$.
\end{proof}
\fi




\iffalse
HAL THIS WASNT DONE, PROBABLY NOT NEEDED, SEE DEF'N OF DUALS BELOW

We now define the blossom
forest at the completion of our construction.
Let $\b G.$ be the graph formed by contracting all blossoms
of a blossom forest \B..
\B.
is {\em complete} if
every vertex of $G$ is in some blossom, and
 the nonloop edges of \b G.
form a spanning tree (with no parallel edges)
where every edge $uv$ belongs
to $I(u)\oplus I(v)$.
\fi

\subsection{Deriving the dual variables}
\label{FDeriveDualsSec}
We first define %start by specifying
the %odd pairs and
dual variables.
Let
\B. be the final blossom forest of our construction.
The term ``blossom'' always refers to a blossom of \B..
Take any blossom $B$ in \B..
$p(B)$ denotes the parent of
$B$ in \B..

Recall that $\o U(B)$
contains an original edge $uv\notin F_u \oplus F_v$ in its circuit
(Lemma \ref{BadCycleLemma}\xii).
 So $\o U(B)$  satisfies the hypothesis of
 Lemma \ref{WeightLemma}\xiii.
% applies to $\o U(B)$.
Applying this lemma
repeatedly shows
$\o U(B)$ is the image of a $2f$-unifactor in $G$, which we denote
as $U(B)$.
We illustrate by noting the weights $\o w(\o U(B))$
and  $w(U(B))$ for Fig.\ref{FContractFig}:
These values are respectively 4 and 4 for (a), $3-2W_1$ and 3 for (b),
$2-2W_1-2W_2$ and 2 for (c).



The reader should heed the following remark, even though
it is not needed in the formal proof.
As stated
above $I(B)$ consists of the edges of $\o U(B)$ that are
incident to $\o V(B)$.
Equivalently $I(B)$ is  the set of all edges of $U(B)$ incident to
$V(B)$.
But $I(B)$ need not be the set of incident edges
of the elementary blossom of $U(B)$. The reason is
that the circuit of $U(B)$ needn't span $V(B_i)$ for $B_i$
a child  of $B$.
For instance in Fig.\ref{NonLamFig}(b),
$V(B_2)=\{a,b,c\}$
and the circuit of $U(B_1)$ is $\{c,d,e\}$.
(In contrast in
Fig.\ref{FContractFig} for
$B$
the blossom of (c), with child blossom $\alpha$,
$U(B)$ spans the entirety of $\alpha=\{b,c,d,e,f\}$.)



For simplicity we refer to the odd pair
$(V(B),I(B))$
as $B$,
and we will shorten $z((V(B), I(B))$ $z(B)$.
Define
%\[
\begin{equation}
\label{DualDefnEqn}
\begin{array}{lcll}
y(v)&=&-w(F_ v)\hspace{102pt}v \in V,\\
%\end{array}\\
%\]
%\[
%z(G)&=&\zeta(G)\\
%z(B) &= &\zeta(B)-\zeta(p(B))&B \mbox{ a blossom }\ne G.
%\begin{array}{lcll}
z(B) &= &
\left\{
\begin{array}{ll}
w(U(B)) &\text{$B$ a root of \B.},\\
w(U(B))-w(U(p(B)))&B \mbox{ a nonroot and nonleaf,}\\
0&\mbox{otherwise.}
\end{array}
\right.
\end{array}
%\]
\end{equation}
Note these duals are defined on $G$ (but not the contracted graphs \b G.).
Also in this definition $w$ denotes the given
function on $G$ with the perturbations
$\epsilon^i$ omitted, i.e.,  we  set $\epsilon $ to 0
in any  context dealing with given weights.
The duals of
Fig.\ref{FExampleFig}(b) illustrate these formulas:
$y$ values come from
Fig.\ref{PerturbationsFig}.
$z$ is computed using the weights $w(U(B))$ noted above from
Fig.\ref{FContractFig}.


Clearly
any blossom $B$ has
\begin{equation}
\label{zEqn}
w(U(B)) =  z\set{C} {V(B)\con V(C)}.
\end{equation}

Observe that $z(B)\ge 0$ for any nonroot blossom $B$:
Lemma \ref{WeightLemma}\iii
shows $U(p(B))$ comes from
an irredundant unifactor in $\b G.(B)$.
So it weighs
less than $U(B)$ in $\b G.(B)$.
Now applying
 Lemma \ref{WeightLemma}\iii repeatedly
shows it weighs less than $U(B)$ in $G$, i.e.,
$w(U(p(B)) \le w(U(B))$ as desired.

Now consider a root blossom $B$.
$z(B)$ is certainly nonnegative if
all weights in $G$ are nonnegative.
We can assume this wlog, since the number of edges in
an $\fs. v$-factor is fixed.
Alternatively it can be seen from Lemma \ref{EndLemma}
that {\em every} $\fs.v$-factor
respects every root blossom of \B.. (The final graph has a unique
$\fs. v$-factor, since the symmetric difference of two
$\fs. v$-factors consists of cycles.)
So nonnegativity of $z(B)$ is not required in
the upperbounding equation (\ref{fFactorDualEqn}).

\iffalse
hal, here is a lemma i was going to include:
Let \bar G be the final graph as described in Lemma \ref{EndLemma}.
\i every $\fs. v$-perturbation has a unique $\fs. v$-factor in
\b G..

\ii every such factor respects every blossom of \bar G.

iii for any v \in V, any $\fs. v$-factor in G respects every root blossom

prove by showing it for a leaf, then a vertex whose neighbors are all leaves,
etc

but the above symmetric difference idea may be better
\fi

The duals $y,z$ and blossom forest \B. form an
optimum $f$-factor structure.
The optimum $f$-factor structure
is defined just like the optimum matching structure, and the details are
tedious. Instead of presenting them we will be content to
prove that our duals are optimum
as specified in Definition \ref{CritOptDualsDefn}.

\iffalse
An {\em optimum matching structure} for an $f$-critical graph
consists of a
  blossom forest \B.
that satisfies the termination condition of
Lemma \ref{EndLemma},
plus dual functions $y,z$,
that make every $C, CH$ and $I$ edge of \B. underrated,
all other edges dominated, and $z$ nonzero only
on \B..
There is an obvious analog of the procedure
$blossom\_match$ that allows us to construct any maximum $f_v$ or
$f^v$ -perturbation. We omit the tedious details.
Instead the proof below shows our maximum $\sF. v$-factors
respect each blossom of \B., thereby establishing optimality of our duals.
\fi

\begin{theorem}
\label{fTheorem}
The duals $y,z$ are optimum for any
$f$-critical graph $G$.
\end{theorem}

\begin{proof}
We need one more notation: For a vertex $v$, let $B_v$ be the minimal
blossom containing $v$ in its circuit. The above discussion shows
that in $G$,
$U(B_v)$ is the maximum weight unifactor containing $v$ in its circuit.
So
\[F_v+F^v=U(B_v).
\]

Let $uv$ be an edge of $G$. %(So $u$ and $v$ are vertices of $G$.)
We will verify the correct relation between
 $\H{yz}(uv)$ and  $w(uv)$.

\yclaim 1 {\it The duals are tight on any edge $uv \in F_v- F_u$.}

\iffalse
$uv\notin C(B_v)$, since $F_v$ omits the two edges $\delta(v)\cap B_v$.
Every maximum perturbation $\Fs. x$, $x \in V(B_v)$
contains the same edges of $\gamma(B_v)-C(B_v)$, i.e., $INT(B)$.
So $uv \in F_v-F_u$ implies $u\notin V(B)$.
\fi

%By definition $v\in C(B_v)$. So
Corollary \ref{LoopCor}\iii
shows $F_u=F^v-uv$.
So $F_u+F_v+uv=F^v+F_v=U(B_v)$.
 Taking weights
shows $w(uv)=w(U(B_v)) +y(u)+y(v)$.
Lemma \ref{I(B)Lemma} shows
$uv$ is covered by the ancestors of $B_v$ and no other
blossoms. So
(\ref{zEqn})
implies tightness.
\ecproof

Henceforth
 assume  $uv\notin F_u\oplus F_v$ (Claim 1).
Thus $uv$ belongs to some unifactor
(Corollary \ref{UnifactorCor}\i and \xii)
and
some blossom $B$ has
$u,v\in V(B)$. Fix
$B$ as the nearest common ancestor of $u$ and $v$
in \B..  $uv$ belongs to either $C(B)$ or $CH(B)$
or to no circuit or chord set of any blossom.
Claims 2--4 treat these three cases respectively.
In these claims
$\bar u$  and $\bar v$
denote
the image of $u$  and $v$ in
$\b G.(B)$, respectively.

\yclaim 2 {\it The duals are tight on any edge $uv\in
C(B)$.}

$\o U (B)$ is the maximum unifactor in $\b G.(B)$ containing
$\bar u \bar v$ in its circuit.
Applying  Lemma \ref{WeightLemma}\iii repeatedly
shows $U(B)$ is the maximum unifactor
in $G$ containing $uv$ in its circuit.
We need only check the two cases below.

\case {$uv \notin F_u\cup F_v$}
Corollary \ref{UnifactorCor}\i shows
$U(B) =F_u+F_v+uv$. Taking weights
shows $w(U(B)) +y(u)+y(v)= w(uv)$.
Lemma \ref{I(B)Lemma} shows
$uv$ is covered by the ancestors of $B$ and no other
blossoms.
Applying (\ref{zEqn}) shows tightness.


\case {$uv \in F_u\cap F_v$}
Corollary \ref{UnifactorCor}\ii shows
$U(B) =F^u+F^v-uv$ and taking weights gives
\[w(U(B)) = w(F^u)+w(F^v)-w(uv).
\]
Adding and subtracting $w(F_u)+w(F_v)$ on the right, and
rearranging,  gives
\[
w(uv)= w(U(B_u))+w(U(B_v))-w(U(B))-w(F_u)-w(F_v).
\]
Since $uv\in F_u\cap F_v$,
Lemma \ref{I(B)Lemma} shows
the blossoms covering
$uv$ are  the ancestors of  $B_u$ or $B_v$
(and no others).
Recall $B$ is  the nearest common ancestor
of $u$ and $v$.
Applying (\ref{zEqn}) to $B_u, B_v$ and $B$
shows
$w(U(B_u))+w(U(B_v))-w(U(B))
 =  z\set{C} {\text{blossom $C$ covers $uv$}}$.
With the last displayed equation this gives tightness.
\ecproof

\yclaim 3 {\it The duals underrate any edge $uv\in CH(B)$.}

$\o U(B)$ does not contain $\bar u \bar v$ in its circuit.
So let $\o T$ be the maximum  irredundant unifactor containing $\bar u \bar v$
in its circuit
in $\b G.(B)$. Obviously $\o T$ weighs less than $\o U(B)$.
Lemma \ref{WeightLemma}\iii
shows $T$, the maximum irredundant unifactor
in $G$ containing $uv$ in its circuit, weighs less than $U(B)$.

The hypothesis of Claim 3 also shows $\bar u \bar v \in
F_{\bar u}\cap F_{\bar v}$, by
Lemma \ref{BlossomUnifactorLemma}.
%Lemmas \ref{UnifactorLemma} and \ref{BlossomUnifactorLemma}.
Using Lemma \ref{WeightLemma}\xi--\ii repeatedly shows
$uv\in  F_u\cap F_v$.
Corollary \ref{UnifactorCor}\ii shows
$T=F^u+F^v-uv$.
Taking weights shows
\[w(U(B))\ge w(T) = w(F^u)+w(F^v)-w(uv).
\]
Now the argument follows the second case of Claim 2, with
inequality rather than equality.
\ecproof

\iffalse
As before adding and subtracting $w(F_u)+w(F_v)$ on the right
and rearranging gives $w(uv)\ge w(B_u)+w(B_v)-w(U(B))-w(F_u)-w(F_v)$.
Now the argument follows Claim 2.
\fi

\yclaim 4 {\it The duals dominate any edge $uv\notin
C(B)\cup CH(B)$.}

Since $B$ is the nearest common ancestor of $u$ and $v$, the
hypothesis of Claim 4 implies $\bar u \bar v \notin \o U(B)$.  Exactly
as in Claim 3 we get that $T$, the maximum irredundant unifactor in
$G$ containing $uv$ in its circuit, weighs less than $U(B)$.

\iffalse
, by Lemmas \ref{UnifactorLemma} and \ref{BlossomUnifactorLemma}.
Using Lemma \ref{WeightLemma}\xi--\ii repeatedly shows
\fi

Similar to  Claim 3,
$\bar u \bar v \notin \o U(B)$ implies $\bar u \bar v \notin
F_{\bar u}\cup F_{\bar v}$ and $uv\notin  F_u\cup F_v$.
Corollary \ref{UnifactorCor}\i shows
$T=F_u+F_v+uv$.
Taking weights shows $w(U(B))\ge w(T) = w(F_u)+w(F_v)+w(uv)$ as desired.
\ecproof

To complete the proof take
any maximum perturbation $\Fs. v$, $v\in V$.
We will show $\Fs. v$ and $y,z$ satisfy the optimality conditions
of Section \ref{fFactorReviewSec}.
$\Fs. v$ consists of edges in sets $C(B), CH(B)$ and $I(B)$
(Definition \ref{BTreeDfn}, Lemma
%s \ref{UnifactorLemma} and
 \ref{BlossomUnifactorLemma}). These edges are underrated (Claims 1--3). The remaining
edges are dominated (Claims 1,2,4).


Finally we must show $\Fs. v$ respects each pair $(V(B),I(B))$ of our duals.
$\Fs. {\bar v}$ respects $(\o V(B),I(B))$ in graph $\b G.(B)$
(Corollary \ref{RespectCor},
 Lemma \ref{WeightLemma}\xi--\xii).
Apply Lemma \ref{RespectLemma}
%(actually the paragraph following it)
to graph $\b G.(B)$
to get $\Fs. {\bar v} \cap \delta(\o V(B))$.
$\Fs. {v} \cap \delta( V(B))$ is the same set,
 in graph $G$.
So applying Lemma \ref{RespectLemma}
in graph $G$  shows
$\Fs. v$ respects $(V(B), I(B))$.

 Thus Definition \ref{CritOptDualsDefn}
 is satisfied and $y,z$ is an optimum dual pair
for the critical graph $G$.
\end{proof}


Now consider a graph $G$ that has an $f$-factor $F$.
(If a vertex has $f(v)=0$ it is irrelevant so delete it.)
Let $G^+$ be $G$ with an additional vertex $s$ and additional edges
$sv,\ v \in V$ plus loop $ss$, all having  weight 0.
Extend $f$ by setting $f(s)=1$.
$G^+$ is critical: For vertex $v\in V$ with
edge $vv'  \in F,\ F-vv' +v' s$ is an $f_v$-factor,
$F+vs$ is an $f^v$-factor,
$F$ and $F+ss$ are respectively $f_s$  and $f^s$ -factors.
So the theorem  gives an optimum structured factor on $G^+$.
Thus we have
optimum duals for an $f_s$-factor  on $G^+$,
i.e., an $f$-factor.
We can delete $s$ to consider these duals defined on $G$.
(A pair $(C,I)$ with positive $z$ and $s\in C$ will no
longer be an odd pair. Such pairs are needed in the standard
integral duals \cite[Ch.32]{S}.)

Regarding uniqueness of the duals,
as in previous sections the
function $y=-w(F_v)$
is canonical: (\ref{fDualEqn}) shows
that any optimum duals $y,z$ for a critical graph
satisfy $(y,z)V-y(v)=w(F_v)$.
The $z$ function is more complex and is analyzed in
Section \ref{CanonSec}.



\iffalse

For an edge $uv\notin F_u\cap F_v$ let
$\zeta(uv) =w(F_u) + w(F_v)+w(uv)$ be the weight of the
maximum $2f$-unifactor cotaining $uv$ in its circuit.

lemma. Let $\zeta^*$ be the maximum weight of a $2f$-unifactor.
Thus $\zeta^*=\max \set {\zeta(v)} {v\in V}$.

Let $\zeta(v)=w(F_v) + w(F^v)$ be the weight of the unifactor of the
lemma. Let $\zeta^*$ be the maximum weight of a $2f$-unifactor.
Thus $\zeta^*=\max \set {\zeta(v)} {v\in V}$.
\fi

\fi

\fi %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Let us now describe an idea of efficient procedure for constructing generalized shortest path tree.
%This should be seen as a specialization of procedure described in Section~\ref{fFactorSec} for $f$-factors.
%We cannot use the procedure directly as described above, because in algorithms we cannot use
%with perturbed edge weights (our weights are integral). We need to work on
%unperturbed edge weights. Let us define the quantity $\zeta_o(uv) = w(P_u)+ w(P_v)+ w(uv)$ over
%original weights. The subgraph $H$ with minimum $\zeta_o$ value does not need to be a simple cycle
%anymore. It can have a more complex structure. However, we can look on $H$ over perturbed edge weighs and see that $H$
%contains a cycle of minimum $\zeta$ value. After shrinking this cycle, we can find another cycle of minimum $\zeta$.
%This implies that $H$ has an ear-decomposition and is $2$-edge connected. Moreover all edges
%with minimum $\zeta_o$ values are tight, so every ear-decomposition of $H$ is equivalent.
%Hence, in the shrinking procedure we find an ear-decomposition of $H$ (this can be done in $O(|E(H)|)$ time
%using greedy algorithm), and then shrink ears one by one. Observe that when we are given weights
% $w(P_v)$ this shrinking procedure can be executed in $O(m \log n)$ time.
%Moreover, the weights $w(P_v)$ can be computed in $O(Wn^{\omega})$ time as given in Section~\ref{sec:weights}.
%Hence, we obtain an $O(Wn^{\omega})$ time algorithm for computing the generalized shortest tree structure.
%
%Finally, we observe that by using the combinatoric interpretation of the related $2$-factor problem (see next section for details), we
%can relate the values $w(P_v)$ to the dual variables. This $2$-factor problem can be efficiently reduced to $1$-factor problem using reduction by Edmonds~\cite{Edmonds67}. The $O(n(m+n\log n))$ time algorithm~\cite{gabow-90} and the $O(\sqrt{n \alpha(m,n)\log n}\ m \log (nW))$ time algorithm~\cite{gt91} for finding $1$-factors solve the dual problem as well. Hence, this solution to the dual
%can be used to obtain $w(P_v)$ and construct the generalized shortest path structure within the same time bounds.
%
%
%


\iffalse
We extend the  ``respects'' relation to the current context.
%(We will mimic the definition of $p(v,N)$ in the gsp-tree.)
A vertex $x$ {\em respects} a node  $C,cc'$ of \T.
if either
$x\in V(C)$ and $P_x=C_x,P_c$; furthermore $P_c$ begins with edge
$cc'$ and is otherwise disjoint from $V(C)$;
or
$x\notin V(C)$ and
either $V(P_x)\cap V(C)=\emptyset$ or
$E(P_x)\cap
(\gamma(C)+ cc')$ equals $C_y+cc'$ for  some $y\in V(C)$.
It is easy to see this definition is consistent with the previous definition
for $x$ respecting a p-cycle of $G$.
\fi

\iffalse
%In the graph $G$ let $S$ be a cycle or a $vt$-path, for an arbitrary $v$.
A subgraph $S$  of $G$ {\em respects} a p-cycle $C,cc'$ of \C.
%(or $C,bb'$) of $G$
if either $V(S)\cap V(C)=\emptyset$ or
$E(S)\cap
(\gamma(C)+ cc')$ equals $C_y+cc'$ for  some $y\in V(C)$.
%$S$ respects \C. if it respects each p-cycle of \C..
%that was shrunk in the construction of $\o G$.
\fi







%=====================
\iffalse
For clarity we use the notation $P_{\o z,H}$, for $z\in V(G)$ and $H$ a contraction
of $G$, denote the shortest-path in $H$ from the image of $z$
to $t$.

A vertex $x\in V(G)$ {\em respects} a p-cycle if either $x\in C$ and $P_x$ is
an $xt$-path in the p-cycle, or $x\notin C$ and $P_x$ either contains
no vertex of $C$ or it contains exactly the same edges of $\gamma(C)+
cc'$ as some $P_y$, $y\in C$.

A vertex $x\in V(G)$ {\em respects} \C.  if either for some $C,cc'$ in
\C., $x\in V(C)$

 and $P_x$ is the minimum-weight $xc$-path in $C$, followed by $P_c$;
 for each $C,cc'$ in \C., $P_c$ begins with edge $cc'$;the p-cycle, or
 $x\notin C$ and $P_x$ either contains no vertex of $C$ or it contains
 exactly the same edges of $\gamma(C)+ cc'$ as some $P_y$, $y\in C$.

We extend the  ``respect'' relation to $\o G$.
We begin by essentially repeating the original definition
in this context:

A vertex $x\in V(G)$ respects \C. if
it respects each of the p-cycles that get shrunk in the formation of
the graph $\o G$ for \C..
(More precisely the image of $x$ in the current graph respects the p-cycle.)

We extend the notion of  ``respects'' to the current context, in both $G$
and $\o G$.
In the graph $G$ let $S$ be a cycle or a $vt$-path, for an arbitrary $v$.
$S$  {\em respects} a p-cycle $C,cc'$ of \C.
%(or $C,bb'$) of $G$
if either $V(S)\cap V(C)=\emptyset$ or $E(S)\cap
(\gamma(C)+ cc')$ equals $C_y+cc'$ for  some $y\in V(C)$.  $S$
respects \C. if it respects each p-cycle of \C..
%that was shrunk in the construction of $\o G$.
It is easy to see this definition is consistent with the previous definition
for $P_x$ respecting a single p-cycle of $G$.

to
be  unique. This is automatic if $\o S$
is a cycle, or
a $vt$-path for $v\notin V(C)$. (For such subgraphs,
any $C,cc'$ of \C. that is in the subgraph $\o S$ is on 2 edges of $\o S$,
$cc'$ and another edge that determines the vertex $y$ in the definition of respect.)
In the remaining case
$v$ is a contracted vertex,
say for $C,cc'$. We require the preimage to be a $ct$-path. This makes
the preimage of $\o S$ unique.
\fi

\iffalse
Consider a contracted vertex Let \C.
Suppose some cycle C,cc' of \C. belongs to a cycle C' of \o G
Let e,f be the edges of \delta(C)in C'
If e,f \ne cc'then C' does not respect \C.
\Delta(
x_i,y_i }\ge \omega/2)
\fi

\iffalse
To show this procedure is correct we first analyze the loop.
We show that for each iteration,

(a) properties P1--P3 hold at the
start of the iteration;

(b) every shortest path $P_x$, $x\in V(G)$, respects every node of (the current)  \T..

In the first iteration (a) holds since the given graph is conservative
and P2--P3 are tautologies.  Now consider an
arbitrary iteration that starts with (a) true.  We show (b) holds, and
(a) holds at the start of the next iteration.

The current graph $\o G$ is conservative, so Lemma \ref{sp2.2} shows
the p-cycle $C,cc'$ of the loop exists.
(The weight of the p-cycle is given by \eqref{WeightSEqn}.)
To prove (b) we must show every $P_x$
respects $C$. Let
$\o x$ be the image of $x$ in $\o G$.
\iffalse
Suppose  $x\in V(C)$. Lemma \ref{sp2.2}\ii shows $\o x$ respects $C$ in $\o G$.
Extend this to $x$ using
P2, and (b) for $x$ and the children of \T..
Next suppose  $x\notin V(C)$.
\fi

Lemma \ref{spRespectLemma} shows $P_{\o x}$ respects $C$ in $\o G$.
P2 shows that in $\o G$, %(assuming $P_{\o x}$ intersects $C$)
$P_x$ contains the same edges of
$\gamma(C)+cc'$ %consists of the edges of
as $P_{\o x}$. In addition, for each child $C'$ of $C$ in \T.
that belongs to $P_{\o x}$, $P_x$ contains the minimum-weight path
in $E(G)\cap \gamma(C')$ joining the appropriate edges of $P_{\o x}$ (by (b)).
This shows
$P_x$ respects $C$.

%Extend this to $P_x$ using P2, and (b) for $P_x$ and the children of \T..

For (a),
Lemma \ref{spContractLemma} shows P1--P3 continue to hold.
This completes the inductive argument.

It is easy to see that (b) also holds if a tree node is
added to \T. when the loop halts.
\fi

\iffalse

Consider an arbtirary edge $uv$. Let $N_0$ be the minimal node
of \T. that covers $uv$. So $uv$  is covered by the ancestors of $N_0$
(and no other nodes).
{}

\zeta(uv)=\ge \zeta^*
d(u)+d(v)+w(uv)\ge \sum \set {z(N)} {N \text{ covers }uv},


Every edge $uv\in E_\ell(G)$ satisfies
\begin{equation}
\label
d(u)+d(v)+w(uv)\ge \sum \set {z(N)} {N \text{ covers }uv},
\end{equation}
with equality holding for every edge of
%in every subgraph $E(N)$ and every loop $xx$.
$\bigcup \set{E(N)}{N \text{ a node of \T.}}$.
\fi
\iffalse

\begin{lemma}
\i Let $C'$ be a cycle of $\o G$.  If $C'$ respects \C. then
$w'(C')=w(C)$ for $C$ the preimage of $C'$.  If $C'$ does not respect
\C.  then $w'(C')\ge \omega$.

\ii Let $P'$ be a $vt$-path in $\o G$. If $P'$ does not respect \C. then
$w'(P')\ge \omega$.  If $P'$ respects \C. let $P$ be the preimage of
$P'$.  If $v$ is a vertex of $G$ then $w'(P')=w(P)$.  If $v$ is a
contracted vertex then $w'(P')=w(P)-\omega$.

\iii Let $uv$ be an edge of $\o G$.  If $uv \notin P_u\oplus P_v$ then
$\zeta'(uv)=\zeta(uv)$.  If $uv \in P_u-P_v$ then $\zeta'(uv)$ is
either $\zeta(uv)$ (if $u$ is a vertex of $\o G$) or $\zeta(uv)-2\omega$
(if $u$ is a contracted vertex of $\o G$).
\end{lemma}


\iffalse

If $x'$ is a vertex of $G$
then $P'_{x'}$ is the image of$P_x$.
If $x'$ is a contracted vertex of $\o G$, say for $C,bb'$,
then  $P'_{x'}$ is the image of$P_b$.
 (in $G$), then the image of $P_x$ in $\o G$. is the imag
\fi


\begin{proof}
Let
$e_1$ and $e_2$ be edges of $\o G$ incident to a common vertex $x$ of $\o G$.
If $x$ is a vertex of $G$ then
\[\Delta(e_1,x)+\Delta(e_2,x)=0.
\]
Suppose $x$ is a contracted vertex.
$\o C$ be a contracted vertex of $\o G$, and
For $i=1,2$ let  $e_i=x_iy_i$ with $x_i\in V(C)$.
If
$e_1,e_2$ respects $C$ then wlog the p-cycle corresponds to $C,e_2$.
Then
\[\Delta(e_1,x_1)+\Delta(e_2,x_2)=w(Q_{x_1}).
\]
In the remaining case,
i.e., $e_1,e_2$ does not respect $C$,
\[\Delta(e_1,x_1)+\Delta(e_2,x_2)\ge \omega/2+\omega/2=\omega.
\]

It is easy to see these 3 relations imply the lemma.
\end{proof}

\iffalse
Consider a contracted vertex Let \C.
Suppose some cycle C,bb' of \C. belongs to a cycle C' of \o G
Let e,f be the edges of \delta(C)in C'
If e,f \ne bb'then C' does not respect \C.
\Delta(
x_i,y_i }\ge \omega/2)
\fi



Part \i shows
$\o G$ is conservative if $G$ is.
Part \ii shows the shortest-paths $P_x$
are the same in $G$ and $\o G$. More precisely,
let $P_x$ ($P'_x$) denote a shortest path in $G$ ($\o G$), respectively.
Let $x'$ be a vertex $\o G$.
$P'_{x'}$ is the image of $P_y$ for every vertex $y$ of $G$ that
is in $x'$. (There is $>1$ $y$ iff $x'$ is a contracted vertex.)
These properties, plus those of the lemma, imply..
\fi



